Latent Outlier Exposure for Anomaly Detection with Contaminated Data

Anomaly detection aims at identifying data points that show systematic deviations from the majority of data in an unlabeled dataset. A common assumption is that clean training data (free of anomalies) is available, which is often violated in practice. We propose a strategy for training an anomaly detector in the presence of unlabeled anomalies that is compatible with a broad class of models. The idea is to jointly infer binary labels to each datum (normal vs. anomalous) while updating the model parameters. Inspired by outlier exposure (Hendrycks et al., 2018) that considers synthetically created, labeled anomalies, we thereby use a combination of two losses that share parameters: one for the normal and one for the anomalous data. We then iteratively proceed with block coordinate updates on the parameters and the most likely (latent) labels. Our experiments with several backbone models on three image datasets, 30 tabular data sets, and a video anomaly detection benchmark showed consistent and significant improvements over the baselines.

==> Latent Outlier Exposure-ICML2022/acknowledgment.tex <==
\section*{Acknowledgements}
Stephan Mandt acknowledges support by the National Science Foundation (NSF) under the NSF CAREER Award 2047418; NSF Grants 1928718, 2003237 and 2007719; the Department of Energy under grant DE-SC0022331, as well as gifts from Intel, Disney, and Qualcomm. This material is in part based upon work supported by the Defense Advanced Research Projects Agency (DARPA) under Contract No. HR001120C0021. Any opinions, findings and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of DARPA. 
Marius Kloft acknowledges support by the Carl-Zeiss Foundation, the DFG awards KL 2698/2-1 and KL 2698/5-1, and the BMBF awards 01$|$S18051A, 03$|$B0770E, and 01$|$S21010C.
We thank Sam Showalter for providing helpful feedback on our manuscript.

The Bosch Group is carbon neutral. Administration, manufacturing and research activities do no longer leave a carbon footprint. This also includes GPU clusters on which the experiments have been performed.

==> Latent Outlier Exposure-ICML2022/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We propose Latent Outlier Exposure (\gls{loe}): a domain-independent approach for training anomaly detectors on a dataset contaminated by unidentified anomalies. During training, \gls{loe} jointly infers anomalous data in the training set while updating its parameters by solving a mixed continuous-discrete optimization problem; iteratively updating the model and its predicted anomalies. Similar to outlier exposure \citep{hendrycks2018deep}, \gls{loe} extracts a learning signal from both normal and abnormal samples by considering a combination of two losses for both normal and (assumed) abnormal data, respectively. Our approach can be applied to a variety of anomaly detection benchmarks and loss functions. As demonstrated in our comprehensive empirical study, \gls{loe} yields significant performance improvements on all three of image, tabular, and video data. 

==> Latent Outlier Exposure-ICML2022/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
We evaluate our proposed methods and baselines for unsupervised anomaly detection tasks on different data types: synthetic data, tabular data, images, and videos.
The data are contaminated with different anomaly ratios.
%The contamination ratio varies in the unlabeled training set. 
Depending on the data, we study our method in combination with specific backbone models. \Gls{mhrot} applies only to images and \gls{icl} to tabular data. \gls{ntl} can be applied to all data types. 
% Across the experiments, we use the Refine and Blind method mentioned in Section~\ref{sec:related} as our baselines.
% As one baseline, we apply the data refinement idea~\citep{yoon2021self} and name it \textit{Refine}. We also blindly apply the original backbone models on the contaminated training data as another baseline, named \textit{Blind}. 
%Below we first study the properties of different methods on controlled synthetic data. Then we present our major experiments on image, tabular, and video data. 

We have conducted extensive experiments on image, tabular, and video data. For instance, we evaluate our methods on all $30$ tabular datasets of \citet{shenkar2022anomaly}. Our proposed method sets a new state-of-the-art on most datasets. In particular, we show that our method gives robust results even when the contamination ratio is unknown. %, demonstrating the methods' robustness regarding training set contamination, even when the contamination rate is unknown. 
%Finally, we investigate our algorithm's robustness of one hyperparameter -- the contamination ratio $\alpha$, which demonstrates our methods also work well in the case of unknown contamination ratio.

% \subsection{Baselines}
% % Robust-PCA, Robust autoencoders, Data-refinement
% Across all experiments, we employ two baselines that do not utilize anomalies to help training the models. The baselines are either completely blind to anomalies, or drop the perceived anomalies' information. Normally training a model without recognizing anomalies serves as our first baseline. Since this baseline doesn't take any actions to the anomalies in the contaminated training data and is actually blind to the anomalies that exist, we name it \textit{Blind}. Mathematically, Blind sets $y_i=0$ in Eq.~\ref{eq:loe-loss} for all samples. 

% The second baseline filters out anomalies and refines the training data: at every mini-batch update, it first ranks the mini-batch data according to the anomaly scores given current detection model, then removes top $\alpha$ most likely anomalous samples from the mini-batch. The remaining samples performs the model update. We name the second baseline \textit{Refine}, which still follows Alg.~\ref{alg:loe} but removes $\La$ in Eq.~\ref{eq:loe-loss}. Both these two baselines take limited actions to the anomalies. We use them to contrast our proposed methods and highlight the useful information contained in unseen anomalies.
% %contrast our proposed methods that utilize anomalies to guide the model training.

\subsection{Toy Example}
\input{figures/toy_data}
We first analyze the methods in a controlled setup on a synthetic data set. 
%We will show that explicitly incorporating the anomaly loss $\La$ during training encloses the normal data region tightly. 
For the sake of visualization, we created a 2D contaminated data set with a three-component Gaussian mixture. One larger component is used to generate normal samples, while the two smaller components are used to generate the anomalies contaminating the data (see \cref{fig:toy_data}). For simplicity, the backbone anomaly detector is the deep one-class classifier~\citep{ruff2018deep} with radial basis functions. Setting the contamination ratio to $\alpha_0=\alpha=0.1$, we compare the baselines ``Blind'' and ``Refine'' (described in \Cref{sec:related}, detailed in \Cref{app:baseline}) with the proposed \gls{loe}$_H$ and \gls{loe}$_S$ (described in \Cref{sec:method}) and the theoretically optimal \textit{G-truth} method (which uses the ground truth labels). We defer all further training details to \Cref{app:toy}.

\cref{fig:toy_data} shows the results (anomaly-score contour lines after training). %From plot (a) to (e), we gradually upweight the anomaly's guidance strength during training: ignoring anomalies (a, b) $\rightarrow$ exploiting detected anomalies (c, d) $\rightarrow$ utilizing ground truth (e). 
With more latent anomaly information exploited from (a) to (e), the contour lines become increasingly accurate. While (a) ``Blind'' erroneously treats all anomalies as normal, (b) ``Refine'' improves by filtering out some anomalies. (c) \gls{loe}$_S$ and (d) \gls{loe}$_H$ use the anomalies, resulting in a clear separation of anomalies and normal data. \gls{loe}$_H$ leads to more pronounced boundaries than \gls{loe}$_S$, but it is at risk of overfitting, especially when normal samples are incorrectly detected as anomalies  (see our experiments below).  A supervised model with ground-truth labels (``G-truth'') approximately recovers the true contours.

\subsection{Experiments on Image Data}
Anomaly detection on images is especially far developed. We demonstrate \gls{loe}'s benefits when applied to two leading image anomaly detectors as backbone models: \gls{mhrot} and \gls{ntl}. Our experiments are designed to test the hypothesis that \gls{loe} can mitigate the performance drop caused by training on contaminated image data. We experiment with three image datasets: CIFAR-10, Fashion-MNIST, and MVTEC \citep{bergmann2019mvtec}. These have been used in virtually all deep anomaly detection papers published at top-tier venues \citep{ruff2018deep,golan2018deep,hendrycks2019using,bergman2020classification,li2021cutpaste}, and we adopt these papers' experimental protocol here, as detailed below. 
%which apply to two different feature levels of images: the pixel-level raw images and the abstract features of images.

\paragraph{Backbone models and baselines.}
We experiment with \gls{mhrot} and \gls{ntl}. In consistency with previous work \citep{hendrycks2019using}, we train \gls{mhrot} on raw images and \gls{ntl} on features outputted by an encoder pre-trained on ImageNet. We use the official code by the respective authors\footnote{\small\url{https://github.com/hendrycks/ss-ood.git}}\footnote{\small\url{https://github.com/boschresearch/NeuTraL-AD.git}}. \gls{ntl} is built upon the final pooling layer of a pre-trained ResNet152 for CIFAR-10 and F-MNIST (as suggested in \citet{defard2021padim}), and upon the third residual block of a pre-trained WideResNet50 for MVTEC (as suggested in \citet{reiss2021panda}).
Further implementation details of \gls{ntl} are in the \Cref{app:imp}.

Many existing baselines apply either blind updates or a refinement strategy to specific backbone models (see \Cref{sec:related}). However, a recent study showed that many of the classical anomaly detection methods such as autoencoders are no longer on par with modern self-supervised approaches \citep{alvarez2022revealing,hendrycks2019using} and in particular found NTL to perform best among 13 considered models.
For a more competitive and unified comparison with existing baselines in terms of the training strategy,
we hence adopt the two proposed \gls{loe} methods (\Cref{sec:method}) and the two baseline methods ``Blind'' and ``Refine'' (\Cref{sec:related}) to two backbone models.
 %In contrast, several recent papers proposed to build anomaly detectors upon the representations from an encoder pretrained on ImageNet \citep{}. Following this, we build \gls{ntl} on the features from a pretrained encoder to detect anomalous images on CIFAR-10 and Fashion-MNIST, and localize anomalous regions on MVTEC.

\paragraph{Image datasets.}
On CIFAR-10 and F-MNIST, we follow the standard ``one-vs.-rest'' protocol of converting these data into anomaly detection datasets~\citep{ruff2018deep,golan2018deep,hendrycks2019using,bergman2020classification}. We create $C$ anomaly detection tasks (where $C$ is the number of classes), with each task considering one of the classes as normal and the union of all other classes as abnormal. For each task, %we mix a fraction of $\alpha_0$ abnormal samples into the training set.
the training set is a mixture of normal samples and a fraction of $\alpha_0$ abnormal samples.
For MVTEC, we use image features as the model inputs. The features are obtained from the third residual block of a WideResNet50 pre-trained on ImageNet as suggested in \citet{reiss2021panda}.
Since the MVTEC training set contains no anomalies, we contaminate it with artificial anomalies that we create by adding zero-mean Gaussian noise to the features of test set anomalies. We use a large variance for the additive noise (equal to the empirical variance of the anomalous features) to reduce information leakage from the test set into the training set.
%For MVTEC there are no anomalies in the training set. Since we only feed the features of MVTEC images into the anomaly detector and its training process, we add Gaussian noise to the features of anomalies in the test set to generate synthetic anomalies. 
%The generated synthetic anomalies (features) together with the features of normal images compose the contaminated training set for MVTEC. 


\paragraph{Results.}
\input{tables/image_results}
\input{figures/acc_ratio}
\input{tables/small_tabular_results}

We present the experimental results of CIFAR-10 and F-MNIST in \cref{tab:image_results}, where we set the contamination ratio $\alpha_0=\alpha=0.1$. 
The results are reported as the mean and standard deviation of three runs with different model initialization and anomaly samples for the contamination.
The number in the brackets is the average performance difference from the model trained on clean data. 
Our proposed methods consistently outperform the baselines and mitigate the performance drop between the model trained on clean data vs. the same model trained on contaminated data. Specifically, with \gls{ntl}, \gls{loe} significantly improves over the best-performing baseline, ``Refine'', by $1.4\%$ and $3.8\%$ AUC on CIFAR-10 and F-MNIST, respectively. On CIFAR-10, our methods have only $0.8\%$ AUC lower than when training on the normal dataset. When we use another state-of-the-art method \gls{mhrot} on raw images, our \gls{loe} methods outperform the baselines by about $2\%$ AUC on both datasets. 

We also evaluate our methods with \gls{ntl} at various contamination ratios (from $5\%$ to $20\%$) in \cref{fig:acc_ratio} (a) and (b). We can see 1) adding labeled anomalies (G-truth) boosts performance, and 2) among all methods that do not have ground truth labels, the proposed \gls{loe} methods achieve the best performance consistently at all contamination ratios. 

%that adding anomalies and knowing the ground truth labels (G-truth) do help train a better anomaly detector than only relying on the normal data (the point at zero contamination ratio), and 2) that our proposed methods, without ground truth labels, achieve the best performance consistently at all contamination ratios. 

We also experimented on anomaly detection and segmentation on the MVTEC dataset. Results are shown in \cref{tab:mvtec_results}, where we evaluated the methods on two contamination ratios ($10\%$ and $20\%$). Our method improves over the ``Blind'' and ``Refine'' baselines in all experimental settings. 

%Overall, experiments with the image datasets demonstrate the effectiveness  of our proposed methods at a negligible cost in the computation. In the following sections, we will validate our methods on more datasets to show the broad application of \gls{loe}.

\subsection{Experiments on Tabular Data}
Tabular data is another important application area of anomaly detection. Many data sets in the healthcare and cybersecurity domains are tabular.
%We evaluate \gls{loe} on a large amount of tabular datasets. 
%For the unsupervised setup, the unlabeled training set is a mixture of normal samples and anomalies which cover the $(1-\alpha)$ fraction and $\alpha$ fraction of the training set respectively. 
Our empirical study demonstrates that \gls{loe} yields the best performance for two popular backbone models on a comprehensive set of contaminated tabular datasets. 

\paragraph{Tabular datasets.}
We study all 30 tabular datasets used in the empirical analysis of a recent state-of-the-art paper \citep{shenkar2022anomaly}. These include the frequently-studied small-scale Arrhythmia and Thyroid medical datasets, the large-scale cyber intrusion detection datasets KDD and KDDRev, and multi-dimensional point datasets from the outlier detection datasets\footnote{\url{http://odds.cs.stonybrook.edu/}}. We follow the pre-processing and train-test split of the datasets in \citet{shenkar2022anomaly}. To corrupt the training set, we create artificial anomalies by adding zero-mean Gaussian noise to anomalies from the test set. 
We use a large variance for the additive noise (equal to the empirical variance of the anomalies in the test set) to reduce information leakage from the test set into the training set.
%The variance of the noise is the empirical variance of the anomalies in the test set.

\paragraph{Backbone models and baselines.}
We consider two advanced deep anomaly detection methods for tabular data described in \Cref{sec:examples}: \gls{ntl} and \gls{icl}. For \gls{ntl}, we use nine transformations and multi-layer perceptrons for neural transformations and the encoder on all datasets. Further details are provided in \Cref{app:imp}. %We search the best-performed transformations types based on the performance of them trained on clean data.
For \gls{icl}, we use the code provided by the authors.
We implement the proposed \gls{loe} methods (\Cref{sec:method}) and the ``Blind" and ``Refine" baselines (\Cref{sec:related}) with both backbone models. 

\paragraph{Results.}
We report F1-scores for 30 tabular datasets in \cref{tab:tabular_small}. The results are reported as the mean and standard derivation of five runs with different model initializations and random training set split. We set the contamination ratio $\alpha_0=\alpha=0.1$ for all datasets. 
More detailed results, including AUCs and the performance degradation over clean data, are provided in \Cref{app:results} (\cref{tab:tabular_f1,tab:tabular_auc}). 

\gls{loe} outperforms the ``Blind" and ``Refine" baselines consistently. Remarkably, on some datasets, \gls{loe} trained on contaminated data can achieve better results than on clean data (as shown in \cref{tab:tabular_f1}), suggesting that the latent anomalies provide a positive learning signal.  
This effect can be seen when increasing the contamination ratio on the Arrhythmia and Thyroid datasets (\cref{fig:acc_ratio} (c) and (d)). \citet{hendrycks2018deep} noticed a similar phenomenon when adding \emph{labeled} auxiliary outliers; these known anomalies help the model learn better region boundaries for normal data. Our results suggest that even \emph{unlabelled} anomalies, when properly inferred, can improve the performance of an anomaly detector.
Overall, we conclude that \gls{loe} significantly improves the performance of anomaly detection methods on contaminated tabular datasets.
%and is potential to utilize the anomalies hidden in the dataset to offer a positive guidance during training.
%However, even \gls{loe} improves the average results a lot, we observed a large variance of the results on some datasets. For example on Optidigits, \gls{loe} achieve either perfect detection or flipped detection in different runs. A flipped detection at beginning could mislead \gls{loe}.

\input{tables/video_results}
\input{figures/ablation}

\subsection{Experiments on Video Data}
In addition to image and tabular data, we also evaluate our methods on a video frame anomaly detection benchmark also studied in \citep{pang2020self}. The goal is to identify video frames that contain unusual objects or abnormal events. 
%Treating frames as independent and exchangeable results in the sets of video frames that are mixtures of normal and abnormal frames. %The assumption is that the abnormal frames are rare in the video clips. Under this assumption, we contaminated the dataset with a small number of anomalies. 
Experiments show that our methods achieve state-of-the-art performance on this benchmark.

\paragraph{Video dataset.}
We study UCSD Peds1\footnote{
  \url{http://www.svcl.ucsd.edu/projects/anomaly/dataset.htm}
}, a popular benchmark for video anomaly detection. It contains surveillance videos of a pedestrian walkway. Non-pedestrian and unusual behavior is labeled as abnormal. 
% For example, carts and bikers are unexpected in a pedestrian walkway and thus are labeled abnormal.  
The data set contains 34 training video clips and 36 testing video clips, where all frames in the training set are normal and about half of the testing frames are abnormal. We follow the data preprocessing protocol of \citet{pang2020self} for dividing the data into training and test sets. To realize different contamination ratios, we randomly remove some abnormal frames from the training set but the test set is fixed.

% Following~\citet{pang2020self}, we treat each frame i.i.d.and  combine the training and test sets. During training, we feed the model with the full, unlabeled dataset (Tr); during testing, we measure the AUCs of the ROC curve on the full dataset with frame labels (Te). To realize different contamination ratios, we randomly remove some abnormal frames from Tr but hold Te fixed. 

\paragraph{Backbone models and baselines.}
In addition to the ``Blind" and ``Refine'' baselines, we compare to ~\citep{pang2020self} (a ranking-based state-of-the-art method for video frame anomaly detection already described in \cref{sec:related}) and all baselines reported in that paper~\citep{sugiyama2013rapid,liu2012isolation, del2016discriminative, tudor2017unmasking, liu2018classifier}. %All of which yield weaker results. 
%The prior state-of-the-art model ~\citep{pang2020self} iteratively predicts which of the video frames are normal and abnormal while updating the model. 
%the data labels and re-trains the ordinal regressor with the most likely normal and abnormal samples.

% Sp~\citep{sugiyama2013rapid} and iForest~\citep{liu2012isolation} assume that, in the feature space, anomalies are far from normal samples, and they separate anomalies based on a distance metric. Other baselines on video anomaly detection include the discriminative framework~\citep{del2016discriminative}, unmasking framework~\citep{tudor2017unmasking}, and a two-sample test improvement over the unmasking method~\citep{liu2018classifier}. 
%We refer the readers to \citep{pang2020self} for the details of all baselines.

We implement the proposed \gls{loe} methods, the ``Blind'', and the ``Refine'' baselines with \gls{ntl} as the backbone model. We use a pre-trained ResNet50 on ImageNet as a feature extractor, whose output is then sent into an \gls{ntl}. The feature extractor and \gls{ntl} are jointly optimized during training.

\paragraph{Results.}
We report the results in \cref{tab:video_results}. Our soft \gls{loe} method achieves the best performance across different contamination ratios. Our method outperforms Deep Ordinal Regression \citep{pang2020self} by 18.8\% and 9.2\% AUC on the contamination ratios of 10\% and 20\%, respectively. \gls{loe}$_S$ outperforms the ``Blind" and ``Refine" baselines significantly on various contamination ratios.

\subsection{Sensitivity Study}
The hyperparameter $\alpha$ characterizes the assumed fraction of anomalies in our training data. %It is crucial to our approach. 
Here, we evaluate its robustness under different ground truth contamination ratios. 
We run \gls{loe}$_H$ and \gls{loe}$_S$ with \gls{ntl} on CIFAR-10 with varying true anomaly ratios $\alpha_0$ and different hyperparameters~$\alpha$. 
We present the results in a matrix accommodating the two variables. The diagonal values report the results when correctly setting the contamination ratio.

\gls{loe}$_H$ (\cref{fig:ablation} (a)) shows considerable robustness: the method suffers at most $1.4\%$ performance degradation when the hyperparameter $\alpha$ is off by $5\%$, and is always better than ``Blind". It always outperforms ``Refine" (\cref{fig:ablation} (c)) when erroneously setting a smaller $\alpha$ than the true ratio $\alpha_0$.  
\gls{loe}$_S$ (\cref{fig:ablation} (b)) also shows robustness, especially when erroneously setting a larger $\alpha$ than $\alpha_0$. The method is always better than ``Refine" (\cref{fig:ablation} (c)) when the hyperparameter $\alpha$ is off by up to $15\%$, and always outperforms ``Blind".
%For example, \gls{loe}$_S$ is always better than the ``Refine" (\cref{tab:image_results}) when the assumed $\alpha$ is larger than the true ratio $\alpha_0$.
%Compared to the ``Blind", \gls{loe}$_S$ is still not worse if we misspecify the contamination ratios within $[-15\%, 15\%]$ window from the true~ratio. 

%Another interesting observation is that \gls{loe}$_S$ consistently achieves the best performance at the off-diagonal line -- when we deliberately set $5\%$ more than the true $\alpha$.
%We conjecture the robustness of \gls{loe}$_S$ comes from the introduced uncertainty in the $\La$ loss. 


==> Latent Outlier Exposure-ICML2022/figures/ablation.tex <==
\begin{figure*}[t]
%\vspace{-10pt}
    \centering
	\begin{subfigure}[b]{0.28\linewidth}
		\includegraphics[width=\linewidth]{images/LOE-R.pdf}
	\caption{LOE$_H$}
	\end{subfigure}
	\begin{subfigure}[b]{0.28\linewidth}
		\includegraphics[width=\linewidth]{images/LOE-W.pdf}
    \caption{LOE$_S$}
	\end{subfigure}
		\begin{subfigure}[b]{0.28\linewidth}
		\includegraphics[width=\linewidth]{images/refine.pdf}
    \caption{Refine}
	\end{subfigure}
%\vspace{-10pt}
    \caption{A sensitivity study of the robustness of \gls{loe}$_H$, \gls{loe}$_S$, and ``Refine'' to the mis-specified contamination ratio. We evaluate them with \gls{ntl} on CIFAR-10 in terms of AUC. \gls{loe}$_H$ and \gls{loe}$_S$ yield robust results and outperform ``Refine'' in the most cases. }
    \label{fig:ablation}
%\vspace{-10pt}
\end{figure*}

==> Latent Outlier Exposure-ICML2022/figures/acc_ratio.tex <==
\begin{figure*}[t!]
%\vspace{-5pt}
    \centering
    	\begin{subfigure}[b]{0.6\linewidth}
		\includegraphics[width=\linewidth]{images/legend.pdf}
	\end{subfigure}	\\
	\begin{subfigure}[b]{0.245\linewidth}
		\includegraphics[width=\linewidth]{images/cifar10.pdf}
	\caption{CIFAR-10}
	\end{subfigure}
		\begin{subfigure}[b]{0.245\linewidth}
		\includegraphics[width=\linewidth]{images/fmnist.pdf}
	\caption{F-MNIST}
	\end{subfigure}
	\begin{subfigure}[b]{0.245\linewidth}
		\includegraphics[width=\linewidth]{images/arrhythmia.pdf}
    \caption{Arrhythmia}
	\end{subfigure}
	\begin{subfigure}[b]{0.245\linewidth}
		\includegraphics[width=\linewidth]{images/thyroid.pdf}
    \caption{Thyroid}
	\end{subfigure}\\
%\vspace{-10pt}
    \caption{Anomaly detection performance of \gls{ntl} on CIFAR-10, F-MNIST, and two tabular datasets (Arrhythmia and Thyroid) with  $\alpha_0 \in \{5\%, 10\%, 15\%, 20\%\}$. \gls{loe} (ours) consistently outperforms the ``Blind'' and ``Refine'' on various contamination ratios.}
    \label{fig:acc_ratio}
%\vspace{-5pt}
\end{figure*}

==> Latent Outlier Exposure-ICML2022/figures/toy_data.tex <==
\begin{figure*}[t!]
%\vspace{-10pt}
    \centering
    %\includegraphics[width=\linewidth]{images/toy_example_without_unseen_outlier.pdf}
%\vspace{-10pt}
    	\begin{subfigure}[b]{0.33\linewidth}
		\includegraphics[width=\linewidth]{images/legend.png}
	\end{subfigure}	\\
	\begin{subfigure}[b]{0.19\linewidth}
		\includegraphics[width=\linewidth]{images/blind.png}
	\caption{Blind}
	\label{fig:toy_blind}
	\end{subfigure}
		\begin{subfigure}[b]{0.19\linewidth}
		\includegraphics[width=\linewidth]{images/refine.png}
	\caption{Refine}
	\label{fig:toy_refine}
	\end{subfigure}
	\begin{subfigure}[b]{0.19\linewidth}
		\includegraphics[width=\linewidth]{images/loe-s.png}
    \caption{LOE$_{S}$}
    \label{fig:toy_soft}
	\end{subfigure}
	\begin{subfigure}[b]{0.19\linewidth}
		\includegraphics[width=\linewidth]{images/loe-h.png}
    \caption{LOE$_{H}$}
    \label{fig:toy_hard}
	\end{subfigure}
		\begin{subfigure}[b]{0.19\linewidth}
		\includegraphics[width=\linewidth]{images/g-truth.png}
    \caption{G-truth}
    \label{fig:toy_truth}
	\end{subfigure}
		\begin{subfigure}[b]{0.0255\linewidth}
		\includegraphics[width=\linewidth]{images/bar.png}
	\caption*{}
	\end{subfigure}
	\\
    \caption{Deep SVDD trained on 2D synthetic contaminated data (see main text) trained with different methods: \textbf{(a)} ``Blind'' (treats all data as normal), \textbf{(b)} ``Refine'' (filters out some anomalies), \textbf{(c)} LOE$_S$ (proposed, assigns soft labels to anomalies),  \textbf{(d)} LOE$_H$ (proposed, assigns hard labels), \textbf{(e)} supervised anomaly detection with ground truth labels (for reference). \gls{loe} leads to improved region boundaries.} 
    \label{fig:toy_data}
%\vspace{-3pt}
\end{figure*}

==> Latent Outlier Exposure-ICML2022/header.tex <==
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{multirow}
\usepackage{algorithm2e}
\usepackage{glossaries}
\makeatletter
\let\oldmakefirstuc\makefirstuc
\renewcommand*{\makefirstuc}[1]{%
  \def\gls@add@space{}%
  \mfu@capitalisewords#1 \@nil\mfu@endcap
}
\def\mfu@capitalisewords#1 #2\mfu@endcap{%
  \def\mfu@cap@first{#1}%
  \def\mfu@cap@second{#2}%
  \gls@add@space
  \oldmakefirstuc{#1}%
  \def\gls@add@space{ }%
  \ifx\mfu@cap@second\@nnil
    \let\next@mfu@cap\mfu@noop
  \else
    \let\next@mfu@cap\mfu@capitalisewords
  \fi
  \next@mfu@cap#2\mfu@endcap
}
\makeatother

\usepackage{hyperref}
\usepackage[capitalise]{cleveref}
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
\usepackage[accepted]{icml2022}

%% defined commands:
%\newacronym{goad}{GOAD}{classification-based anomaly detection}
\newacronym{mhrot}{MHRot}{multi-head RotNet}
\newacronym{ntl}{NTL}{anomaly detection using neural transformations}
\newacronym{icl}{ICL}{anomaly detection with internal contrastive learning}
\newacronym{loe}{LOE}{latent outlier exposure}

\newcommand{\Ln}{{\mathcal{L}^\theta_n}}
\newcommand{\La}{{\mathcal{L}^\theta_a}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\cq}[1]{{[\color{blue}\textbf{CQ: #1}]}}
\newcommand{\al}[1]{{[\color{orange}\textbf{AL: #1}]}}


==> Latent Outlier Exposure-ICML2022/introduction.tex <==
\section{Introduction}
From industrial fault detection to medical image analysis or financial fraud prevention: Anomaly detection---the task of automatically identifying anomalous data instances without being explicitly taught how anomalies may look like---is critical in industrial and technological applications. 
    
The common approach in deep anomaly detection is to first train a neural network on a large dataset of ``normal" samples minimizing some loss function (such as a deep one-class classifier~\citep{ruff2018deep}) and to then construct an anomaly score from the output of the neural network (typically based on the training loss).  Anomalies are then identified as data points with larger-than-usual anomaly scores and obtained by thresholding the score at particular~values. 
   
A standard assumption in this approach is that clean training data are available to teach the model what ``normal" samples look like \citep{ruff2021unifying}. In reality, this assumption is often violated: datasets are frequently large and uncurated and may already contain some of the anomalies one is hoping to find. For example, a dataset of medical images may already contain cancer images, or datasets of financial transactions could already contain unnoticed fraudulent activity. Naively training an unsupervised anomaly detector on such data may suffer from degraded performance. 
   
In this paper, we introduce a new unsupervised approach to training anomaly detectors on a corrupted dataset. Our approach uses a combination of two coupled losses to extract learning signals from both normal and anomalous data. We stress that these losses do not necessarily have a probabilistic interpretation; rather, many recently proposed self-supervised auxiliary losses can be used \citep{ruff2018deep,hendrycks2019using,qiu2021neural,shenkar2022anomaly}. In order to decide which of the two loss functions to activate for a given datum (normal vs. abnormal), we use a binary latent variable that we jointly infer while updating the model parameters. Training the model thus results in a joint optimization problem over continuous model parameters and binary variables that we solve using alternating updates. During testing, we can use threshold only one of the two loss functions to identify anomalies in constant time. 





%Our idea is as follows. Distinguishing normal from anomalous data by a set of binary labels, we are interested in jointly inferring these labels and updating our model parameters. This leads to a joint optimization problem over continuous model parameters and binary variables that we solve using alternating updates. When updating the binary variables, we hold the model parameters fixed. When performing a gradient step on the model parameters, we hold our assignments into normal and anomalous data fixed. 

%Our approach uses a combination of two losses to extract learning signals from both normal and anomalous data. We stress that these losses do not necessarily have a probabilistic interpretation; rather, many recently proposed self-supervised auxiliary losses can be used \citep{ruff2018deep,hendrycks2019using,qiu2021neural,shenkar2022anomaly}. The two losses resemble the ``Outlier Exposure" approach~\citep{hendrycks2018deep} that trains an anomaly detector in the presence of synthetic, but note that our anomalies are not synthetic but are present in the training data and have to be inferred while training the model. Remarkably, we exploit that even unlabeled anomalies may provide a valuable training signal about their characteristic features~\citep{nigam2000text}. 

%The idea is that even unlabeled anomalies may provide a valuable training signal about abnormal features~\citep{nigam2000text}. The resulting algorithm bears strong similarities to an expectation-maximization (EM) scheme~\citep{dempster1977maximum}, with a few notable differences. First, we infer the labels based on the "normal" part of the loss function, i.e., without the outlier exposure loss.  Second, we soften the label for better performance, allowing the algorithm to be uncertain about its prediction. Interestingly, our analysis shows that the presence of unlabeled outliers in the training data does not necessarily lead to a performance drop over "clean" data, but can in some cases even lead to better performance.
   
Our approach can be applied to a variety of anomaly detection loss functions %\citep{ruff2018deep,hendrycks2019using,qiu2021neural,shenkar2022anomaly} 
and data types, as we demonstrate on tabular, image, and video data. Beyond detection of entire anomalous images, we also consider the problem of anomaly segmentation  which is concerned with finding anomalous regions within an image. Compared to established baselines that either ignore the anomalies or try to iteratively remove them~\citep{yoon2021self}, our approach yields significant performance improvements in all cases. 

The paper is structured as follows. In \Cref{sec:related}, we discuss related work. In \Cref{sec:method}, we introduce our main algorithm, including the involved losses and optimization procedure. Finally, in \Cref{sec:experiments}, we discuss experiments on both image and tabular data and discuss our findings in \Cref{sec:conclusion} \footnote{Code is available at \url{https://github.com/boschresearch/LatentOE-AD.git}}. 
 
%Motivation: the information contained by unlabeled anomalies \citep{nigam2000text}. unlabeled anomalies do contain information about the abnormal features other than the class label. Because of this they can sometimes be used to significantly increase the anomaly detection accuracy in semi-supervised and even unsupervised anomaly detection.

%In unsupervised anomaly detection, the performance of detectors drops as the anomaly ratio increases in the training set.In contrast, in the supervised anomaly detection, the performance of detectors increases as the anomaly ratio increases in the training set, since the ground truth labels provide the correct guidance in the training. In this work, we propose a procedure to estimate and use the unlabeled anomalies in the training to improve the model performance in unsupervised anomaly detection.

==> Latent Outlier Exposure-ICML2022/method.tex <==
\section{Method}
\label{sec:method}
We will start by describing the mathematical foundations of our method. We will then describe our learning algorithm as a block coordinate descent algorithm, providing a theoretical convergence guarantee. Finally, we describe how our approach is applicable in the context of various state-of-the-art deep anomaly detection methods. 

\subsection{Problem Formulation}

\paragraph{Setup.} In this paper, we study the problem of unsupervised (or self-supervised) anomaly detection. We consider a data set of samples $\x_i$; these could either come from a data distribution of ``normal" samples, or could  otherwise come from an unknown corruption process and thus be considered as ``anomalies". For each datum $\x_i$, let $y_i=0$ if the datum is normal, and $y_i=1$ if it is anomalous. We assume that these binary labels are unobserved, both in our training and test sets, and have to be inferred from the data.

In contrast to most anomaly detection setups, we assume that our dataset is \emph{corrupted by anomalies}. That means, we assume that a fraction $(1-\alpha)$ of the data is normal, while its complementary fraction $\alpha$ is anomalous. This corresponds to a more challenging (but arguably more realistic) anomaly detection setup since the training data cannot be assumed to be normal. We treat the assumed contamination ratio $\alpha$ as a hyperparameter in our approach and denote $\alpha_0$ as the ground truth contamination ratio where needed. Note that an assumed contamination ratio is a common hyperparameter in many robust algorithms \citep[e.g.,][]{huber1992robust,huber2011robust}, and we test the robustness of our approach w.r.t. this parameter in \Cref{sec:experiments}.

Our goal is to train a (deep) anomaly detection classifier on such corrupted data based on self-supervised or unsupervised training paradigms (see related work). The challenge thereby is to simultaneously infer the binary labels $y_i$ during training while optimally exploiting this information for training an anomaly detection model. 

\paragraph{Proposed Approach.}
We consider two losses. Similar to most work on deep anomaly detection, we consider a loss function $\Ln(\x)\equiv {\cal L}_n(f_\theta(\x))$ that we aim to minimize over ``normal" data. The function $f_\theta(\x)$ is used to extract features from $\x$, typically based on a self-supervised auxiliary task, see \Cref{sec:examples} for examples. When being trained on only normal data, the trained loss will yield lower values for normal than for anomalous data so that it can be used to construct an anomaly score. 

In addition, we also consider a second loss for anomalies $\La(\x)\equiv {\cal L}_a (f_\theta(\x))$ (the feature extractor $f_\theta(\x)$ is shared). Minimizing this loss on only anomalous data will result in low loss values for anomalies and larger values for normal data. The anomaly loss is designed to have opposite effects as the loss function $\Ln(\x)$. For example, if $\Ln(\x)=||f_\theta(\x)-{\bf c}||^2$ as in Deep SVDD \citep{ruff2018deep} (thus pulling normal data points towards their center), we define $\La(\x) = 1/||f_\theta(\x)-{\bf c}||^2$ (pushing abnormal data away from it) as in \citep{ruff2019deep}. %Examples for other loss functions are provided in Table~\ref{tab:anomaly loss}.  

%\input{tables/negative_losses}

Temporarily assuming that all assignment variables $\y$ were known, consider the joint loss function,
\begin{align}
\label{eq:loe-loss}
    {\cal L}(\theta, \y) = \sum_{i=1}^N (1-y_i) \Ln(\x_i) + y_i \La(\x_i).
\end{align}
This equation resembles the log-likelihood of a probabilistic mixture model, but note that $\Ln(\x_i)$ and $\La(\x_i)$ are not necessarily data log-likelihoods; rather, self-supervised auxiliary losses can be used and often perform better in practice \citep{ruff2018deep, qiu2021neural, nalisnick2018deep}. 

Optimizing Eq.~\ref{eq:loe-loss} over its parameters $\theta$ yields a better anomaly detector than $\Ln$ trained in isolation. By construction of the anomaly loss $\La$, the known anomalies provide an additional training signal to $\Ln$: due to parameter sharing, the labeled anomalies teach $\Ln$ where \emph{not} to expect normal data in feature space. This is the basic idea of Outlier Exposure \citep{hendrycks2018deep}, which constructs artificial \emph{labeled} anomalies for enhanced detection performance. 

Different from Outlier Exposure, we assume that the set of $y_i$ is unobserved, hence \emph{latent}. We therefore term our approach of jointly inferring latent assignment variables $\y$ and learning parameters $\theta$ as \emph{\Gls{loe}}. We show that it leads to competitive performance on training data corrupted by outliers.

\subsection{Optimization problem}
\label{sec:optimization}

\paragraph{``Hard" Latent Outlier Exposure (\gls{loe}$_H$).}
In \gls{loe}, we seek to both optimize both losses' shared parameters $\theta$ while also optimizing the most likely assignment variables $y_i$. Due to our assumption of having a fixed rate of anomalies $\alpha$ in the training data, we introduce a constrained set:
\begin{align}
\label{eq:label-constraint}
    {\cal Y} = \{\y \in \{0,1\}^N: \sum_{i=1}^N y_i = \alpha N\}.
\end{align}
The set describes a ``hard" label assignment; hence the name ``Hard \gls{loe}", which is the default version of our approach.  
\Cref{sec:extension} describes an extension with ``soft" label assignments. Note that we require $\alpha N$ to be an integer. 

Since our goal is to use the losses $\Ln$ and $\La$ to identify and score anomalies, we seek $\Ln(\x_i) - \La(\x_i)$ to be large for anomalies, and $\La(\x_i) - \Ln(\x_i)$ to be large for normal data. Assuming these losses to be optimized over $\theta$, our best guess to identify anomalies is to minimize \cref{eq:loe-loss} over the assignment variables $\y$. Combining this with the constraint  (\cref{eq:label-constraint}) yields the following minimization problem:
\begin{align}
    \label{eq:optimization-problem}
    \min_\theta \min_{\y \in {\cal Y}} \;  {\cal L}(\theta,\y).
\end{align}
As follows, we describe an efficient optimization procedure for the constraint optimization problem. 

\paragraph{Block coordinate descent.} 
The constraint discrete optimization problem has an elegant solution. 

To this end, we consider a sequence of parameters $\theta^t$ and labels $\y^t$ and proceed with alternating updates. To update $\theta$, we simply fix $\y^t$ and minimize ${\cal L}(\theta, \y^t)$ over $\theta$. In practice, we perform a single gradient step (or stochastic gradient step, see below), yielding a partial update. 

To update $\y$ given $\theta^t$, we minimize the same function subject to the constraint (\cref{eq:label-constraint}). To this end, we define training anomaly scores,
\begin{align}
    S_i^{train} = \Ln(\x_i) - \La(\x_i). 
\end{align}
These scores quantify the effect of $y_i$ on minimizing \cref{eq:loe-loss}. We rank these scores and assign the $(1-\alpha)$-quantile of the associated labels $y_i$ to the value $0$, and the remainder to the value $1$. This minimizes the loss function subject to the label constraint. We discuss the sensitivity of our approach to the assumed rate of anomalies $\alpha$ in our experiments section. We stress that our testing anomaly scores will be different (see \Cref{sec:extension}). 

%Intuitively, $s_i$ quantifies the change of the overall loss due to flipping the label $y_i$. Hence, in order to minimize over $y_i$ subject to $\y \in {\cal Y}$, we find permutation indices $\{i_1, ..l.\i_N\}$ such that $s_{i_1}\leq s_{i_1} \leq ... \leq s_{i_N}$ (thus ranking the anomaly scores), and then assign $y_{i_1} = ... = y_{i_{(1-\alpha)N}} = 0$ and $y_{i_{1+(1-\alpha)N}} = ... = y_{i_N}=1$. This scalably solves the discrete constrained optimization problem. 

Assuming that all involved losses are bounded from below, the block coordinate descent converges to a local optimum since every update improves the loss. 

\paragraph{Stochastic optimization.} In practice, we perform stochastic gradient descent on \cref{eq:loe-loss} based on mini-batches. For simplicity and memory efficiency, we impose the label constraint \cref{eq:label-constraint} on each mini-batch and optimize $\theta$ and $\y$ in the same alternating fashion. The induced bias vanishes for large mini-batches. In practice, we found that this approach leads to satisfying results\footnote{Note that an exact mini-batch version of the optimization problem in \cref{eq:optimization-problem} would also be possible, requiring memorization of $\y$ for the whole data set.}.

\Cref{alg:loe} summarizes our approach. 
\input{pseudo_code}

\subsection{Model extension and anomaly detection}
\label{sec:extension}
We first discuss an important extension of our approach and then discuss its usage in anomaly detection.

\paragraph{``Soft'' Latent Outlier Exposure (\gls{loe}$_S$).}
%and an auxiliary loss function $\Ln(\x)$
In practice, the block coordinate descent procedure can be overconfident in assigning $\y$, leading to suboptimal training. To overcome this problem, we also propose a \emph{soft} anomaly scoring approach that we term \emph{Soft} \gls{loe}.  Soft \gls{loe} is very simply implemented by a modified constraint set:
\begin{align}
    {\cal Y}' = \{\y \in \{0,0.5\}^N: \sum_{i=1}^N y_i = 0.5\alpha N\}.
\end{align}
Everything else about the model's training and testing scheme remains the same. 

The consequence of an identified anomaly $y_i=0.5$ is that we minimize an equal combination of both losses, $0.5(\Ln(\x_i) + \La(x_i))$. The interpretation is that the algorithm is uncertain about whether to treat $\x_i$ as a normal or anomalous data point and treats both cases as equally likely. A similar weighting scheme has been proposed for supervised learning in the presence of unlabeled examples \citep{lee2003learning}. In practice, we found the soft scheme to sometimes outperform the hard one (see \Cref{sec:experiments}). 

\paragraph{Anomaly Detection.}
In order to use our approach for finding anomalies in a test set, we could in principle proceed as we did during training and infer the most likely labels as described in \Cref{sec:optimization}. However, in practice we may not want to assume to encounter the same kinds of anomalies that we encountered during training. Hence, we refrain from using $\La$ during testing and score anomalies using only $\Ln$. Note that due to parameter sharing, training $\La$ jointly with $\Ln$ has already led to the desired information transfer between both losses.

Testing is the same for both ``soft" \gls{loe} (\Cref{sec:optimization}) and ``hard" \gls{loe} (\Cref{sec:extension}). We define our testing anomaly score in terms of the ``normal" loss function,
\begin{align}
    S^{test}_i = \Ln(\x_i).
\end{align}
%For predicting anomalies, we then threshold the anomaly score. The threshold should thereby obey our working assumption of a fraction of $\alpha$ anomalous samples among the data. Similar to \citep{yoon2021self}, we search for the optimal threshold $\gamma^\alpha$ by solving
%\begin{align}
%\label{eqn:gamma}
%    \gamma^\alpha = \max \gamma \quad \text{s.th. } \sum_{i=1}^N \mathbbm{1} (S_i^{train}\geq\gamma) \geq \alpha N.
%\end{align}

%\subsection{Preliminaries}
%Self-supervised methods learn the feature extractor and representations by solving an auxiliary task $A$. The learned model and representations can be then used in the downstream tasks including anomaly detection. Specifically, the model is trained by minimizing the loss $\Ln(x)$ on the auxiliary task. A convenient choice of the anomaly score is using the auxiliary loss function as
%\begin{align}
%    S(x):=\mathcal{L}_{A}(x).
%\end{align}
%Given the threshold $\gamma$, the detection is formulated as  
%\begin{align}
%    \hat{y}= 
%\begin{cases}
%    1,& \text{if } S(x) \geq \gamma\\
%    0,& \text{otherwise,}
%\end{cases}
%\end{align}
%where $\hat{y}$ is the predicted label of being an anomaly.
%These methods draw on the simple concept of ``inlier priority''\citep{wang2019effective}, that is, promoting the trained model to generalize better to held-out inliers than outliers.

\subsection{Example loss functions}
\label{sec:examples}
As follows, we review several loss functions that are compatible with our approach. We consider three advanced classes of self-supervised anomaly detection methods. 
These methods are i) \gls{mhrot} \citep{hendrycks2019using}, ii) \gls{ntl} \citep{qiu2021neural}, and iii) \gls{icl} \citep{shenkar2022anomaly}. While no longer being considered as a competitive baseline, we also consider deep SVDD for visualization due to its simplicity.
% approaches have a feature extractor $f(\cdot): \mathcal{X} \rightarrow \mathcal{Z}$ and a set of transformations $\mathcal{T}:=\{T_1,...,T_K \mid T_k(\cdot) : \mathcal{X} \rightarrow \mathcal{X}\}$. 
%They differ in the transformations and the corresponding  auxiliary loss $\mathcal{L}_{A}(x)$. 

\paragraph{Multi-Head RotNet (MHRot).}
\gls{mhrot} \citep{hendrycks2019using} learns a multi-head classifier $f_\theta$ to predict the applied image transformations including rotation, horizontal shift, and vertical shift. We denote $K$ combined transformations as $\{T_{1},...,T_{K}\}$.
The classifier has three softmax heads, each for a classification task $l$, modeling the prediction distribution of a transformed image $p^l(\cdot | f_\theta, T_k(\x))$ (or $p_k^l(\cdot|\x)$ for brevity). % where $l$ denotes the task and the associated head.
%\gls{mhrot} applies self-supervised learning on hand-crafted image transformations including rotation, horizontal shift, and vertical shift. The learner learns to solve three different tasks: 
%one for predicting rotations, one for predicting vertical shifts, one for predicting horizontal shifts. We use the same transformation parameters as  \citet{hendrycks2019using}. We denote all possible combined transformations $T_c(\cdot)$ by ${\cal T}$. Each $T_c$ is associated with labels $\mathbf{t}_c$, denoting which transformation is in use. 
%The model has a softmax head for each task, modeling the predicted transformation distributions $p_c^l(\cdot | f_\theta, T_c(\x))$ (or $p_c^l(\cdot)$ for simplicity) where $l$ denotes the task in consideration.
% one for predicting rotation ($r\in \mathcal{R}\equiv\{0^{\circ}, \pm90^{\circ}, 180^{\circ}\}$), one for predicting vertical shift ($s^v \in \mathcal{S}^v\equiv\{0\text{\,px}, \pm 8\text{\,px}\}$), and one for predicting horizontal shift ($s^h \in \mathcal{S}^h\equiv\{0\text{\,px}, \pm 8\text{\,px}\}$). 
% We define the composition of rotation, vertical shift, and horizontal shift as $T \in {\cal T}\equiv\{r\circ s^v \circ s^h \mid r\in \mathcal{R}, s^v \in \mathcal{S}^v, s^h \in \mathcal{S}^h\}$. We also define the head labels $t^1_c=r_i, t^2_c=s^v_j, t^3_c=s^h_k$ for a specific composed transformation $T_c=r_i\circ s^v_j \circ s^h_k$.
Aiming to predict the correct transformations for normal samples, we maximize the log-likelihoods of the ground truth label $t_k^l$ for each transformation and each head;
% and set $\Ln(\x):=  -\sum_{c=1}^{|\mathcal{T}|}\sum_{l=1}^3 \log p_l(t^l_c | f,T_c(\x))$
for anomalies, we make the predictions evenly distributed by minimizing the cross-entropy from a uniform distribution $\mathcal{U}$ to the prediction distribution, resulting in %The combined loss for a  pair $(\x, y)$ is
% $\La(\x)&: =  \sum_{c=1}^{|\mathcal{T}|}\sum_{l=1}^3 \text{CE}(\mathcal{U}, p_l(\cdot | f,T_c(\x)))$.
\begin{align*}
   % {\cal L}^\theta(\x, y) := 
 %   \sum_{k=1}^{K}\sum_{l=1}^3 
 %       -(1\!-\!y_i)\log p_k^l(t_k^l|\x_i) + y_i\mathcal{H}(\mathcal{U}, p_k^l(\cdot|\x_i))
     \Ln(\x)&:=-\textstyle\sum_{k=1}^{K}\sum_{l=1}^3  \log p_k^l(t_k^l|\x),\nonumber\\ \La(\x)&:=\textstyle\sum_{k=1}^{K}\sum_{l=1}^3 \text{CE}(\mathcal{U}, p_k^l(\cdot|\x))\nonumber
    % \Ln(\x)&:= 
    %  -\sum_{c=1}^{|\mathcal{T}|}\sum_{l=1}^3 \log p_l(t^l_c\mid f,T_c(\x))\\
    %  \La(\x)&: =  \sum_{c=1}^{|\mathcal{T}|}\sum_{l=1}^3 \text{CE}(\mathcal{U}, p_l(\cdot \mid f,T_c(\x)))
\end{align*}
%The first and second terms are  
%$\Ln$ and $\La$, respectively.
\paragraph{Neural Transformation Learning (NTL).}
Rather than using hand-crafted transformations, \gls{ntl} learns $K$ neural transformations $\{T_{\theta,1},...,T_{\theta,K}\}$ and an encoder $f_\theta$ parameterized by $\theta$ from data and uses the learned transformations to detect anomalies. Each neural transformation generates a view $\x_k = T_{\theta,k}(\x)$ of sample $\x$. 
For normal samples, \gls{ntl} encourages each transformation to be similar to the original sample and to be dissimilar from other transformations. To achieve this objective, \gls{ntl} maximizes the normalized probability $p_k=h(\x_k, \x)\big/\big(h(\x_k, \x)+\sum_{l\neq k}h(\x_k, \x_l)\big)$ for each view where $h(\mathbf{a},\mathbf{b}) = \exp (\mathrm{cos}(f_\theta(\mathbf{a}), f_\theta(\mathbf{b}))/ \tau)$ measures the similarity of two views \footnote{
  where $\tau$ is the temperature and $\mathrm{cos}(\mathbf{a},\mathbf{b}) := \mathbf{a}^T \mathbf{b}/ \|\mathbf{a}\| \|\mathbf{b}\|$
}. For anomalies, we ``flip” the objective for normal samples: the model instead pulls the transformations close to each other and pushes them away from the original view, resulting in
% we design $\La$ “inversely” for anomalies to pull the transformations with each other and push them away from the original sample.
%$\mathrm{sim}(a,b)$ can be any similarity measure.
%$\mathrm{sim}(a,b)$ is the cosine similarity as
% Given a similarity function of two views $h(a,b) = \exp (\mathrm{sim}(a, b)/ \tau)$, 
% $\Ln$ and $\La$ are defined with a similarity function of two views $h(a,b) = \exp (\mathrm{sim}(a, b)/ \tau)$ \footnote{where $\tau$ is the temperature and $\mathrm{sim}(a,b) := a^T b/ \|a\| \|b\|$} as %using the the similarity function $h$ as
\begin{align*}
%   \Ln(\x)&:= %-\sum_{k=1}^K \log p_k(x\mid f,\mathcal{T}) \\
%   -\sum_{k=1}^K \log \frac{h(f(\x_k), f(\x))}{h(f(\x_k), f(\x))+\textstyle\sum_{l\neq k}h(f(\x_k), f(\x_l))} \nonumber\\
%   \La(\x) & :=  -\sum_{k=1}^K \log \frac{\sum_{l\neq k}h(f(\x_k), f(\x_l))}{h(f(\x_k), f(\x))+\textstyle\sum_{l\neq k}h(f(\x_k), f(\x_l))} \nonumber
    \Ln(\x):= -\sum_{k=1}^K \log p_k, \quad \La(\x):= -\sum_{k=1}^K \log (1-p_k).
\end{align*}
%Intuitively, the term in the nominator pulls the transformed embeddings close
%to the reference embedding. This encourages the transformed embeddings to preserve relevant semantic information with the reference embedding. The denominator pushes all transformed embeddings away from each other, thereby encouraging diverse transformations.

\paragraph{Internal Contrastive Learning (ICL).}
\gls{icl} is a state-of-the-art \textit{tabular} anomaly detection method \citep{shenkar2022anomaly}. Assuming that the relations between a subset of the features (table columns) and the complementary subset are class-dependent, \gls{icl} is able to learn an anomaly detector by discovering the feature relations for a specific class. %This classifier can be then used to detect anomalies. 
With this in mind, \gls{icl} learns to maximize the mutual information between the two complementary feature subsets, $a(\x)$ and $b(\x)$, in the embedding space. The maximization of the mutual information is equivalent to minimizing a contrastive loss $\Ln(\x):= -\sum_{k=1}^K \log p_k$ on normal samples with $p_k=h(a_k(\x), b_k(\x))\big/\sum_{l=1}^K h(a_l(\x), b_k(\x))$ where $h(a,b) = \exp (\mathrm{cos}(f_\theta(a), g_\theta(b))/ \tau)$ measures the similarity of two feature subsets in the embedding space of two encoders $f_\theta$ and $g_\theta$. For anomalies, we flip the objective as $\La(\x):= -\sum_{k=1}^K \log (1-p_k)$.
% the losses as
% \begin{align*}
%     \Ln(\x) := -\sum_{k=1}^K \log p_k, \quad \La(\x) := -\sum_{k=1}^K \log (1-p_k).
% \end{align*}

% Specifically, \gls{icl} minimizes a  $-\log p_k$ where $p_k=$, which learns two encoders $f$ and $g$ parameterized by $\theta$ to minimize a contrastive learning loss, which equivalently maximizes the mutual information~\citep{}.
% two encoders $f$ and $g$ to align two disjoint sets of features $a_k(\x)$ and $b_k(\x)$ while pushing $b_k(x)$ away from other feature sets $a_l(\x)$ for $l\neq k$. For normal samples, we train the encoders to extract dependencies between non-overlapped features by minimizing a contrastive loss $\Ln$. For anomalies we design $\La$ to align $b_k(x)$ with its overlapped sets. By repeating over $K$ sets $\Ln$ and $\La$ are defined with $h(a,b) = \exp (\mathrm{sim}(a, b))/ \tau)$ as 
% \begin{align*}
%   \Ln(\x)&:= %-\sum_{k=1}^K \log p_k(x\mid f,g,\mathcal{T}) \\
%   -\sum_{k=1}^K \log \frac{h(g(b_k(\x)), f(a_k(\x)))}{\sum_{l=1}^K h(g(b_k(\x)), f(a_l(\x)))} \nonumber\\
%       \La(\x) & := -\sum_{k=1}^K \log \frac{\sum_{l\neq k} h(g(b_k(\x)), f(a_l(\x)))}{\sum_{l=1}^K h(g(b_k(\x)), f(a_l(\x)))}\nonumber
% \end{align*}

%\paragraph{Deep SVDD}
%Deep SVDD learns an encoder $f$ to embed normal samples into a compact hypersphere in the embedding space. $\Ln$ is designed to minimize the distance of the sample to a fixed center in the embedding space. We follow \citet{ruff2019deep} to use   
%\begin{align}
%   \Ln(x)&:= ||f(x)-c||^2 \\
%   \La(x)&:= 1/||f(x)-c||^2 
%\end{align}

\iffalse
\paragraph{Classification-based Anomaly Detection}
\gls{goad} applies hand-crafted transformations to the samples including rotation, shift, and flipping. 
The auxiliary loss is defined as,
\begin{align}
        \mathcal{L}_A(x) &:= -\sum_{k=1}^K \log p_k(x\mid f,\mathcal{T}) \\
        &=-\sum_{k=1}^K \log \frac{\exp(-||f(T_k(x))-c_k||^2)}{\sum_{l=1:K}\exp(-||f(T_l(x))-c_l||^2)}.\nonumber
\end{align}
\fi

%\subsection{Proposed Method}
%We propose a new procedure for the training of self-supervised anomaly detection methods in unsupervised anomaly detection. It estimates the labels of training samples and uses them as the additional guidance in the training iteratively. In order to incorporate the anomalies in the loss function, we extend the loss functions proposed in existing self-supervised anomaly detection methods. Specifically, we define the loss function as
%\begin{align}
%\label{eqn:loss}
%    \mathcal{L} = &-\frac{1}{N}\sum_{i=1}^N\left[(1-\hat{y}_i) \mathcal{L}_{OA}(x_i)+\hat{y}_i \mathcal{L}_{A}(x_i)\right],
%\end{align}
%where $\mathcal{L}_{OA}(x)$ is the auxiliary loss term for the estimated anomalous training samples. While $\mathcal{L}_{A}(x)$ trains the model to perform well on the auxiliary task, $\mathcal{L}_{OA}(x)$ trains the model oppositely. The specific formulation of $\mathcal{L}_{OA}(x)$ is a design choice, and depends on the task at hand and the anomaly detector used. 
%\input{tables/negative_losses}
%Even we define $\mathcal{L}_{OA}$ in \Cref{tab:neg_losses}, other choices can also possible. 
%For example, we can also formulate $\mathcal{L}_{OA}$ for \gls{mhrot} as minimizing the cross-entropy between the uniform distribution and the model distribution as in \citet{hendrycks2018deep}.

%A key ingredient in the loss function is how to estimate the label $\hat{y}_i$.   
%\begin{align}
%\text{Radical:}\quad&\hat{y}_i= 
%\begin{cases}
%    1,& \text{if } S(x_i)\geq \gamma_{mb}\\
%    0,              & \text{otherwise}
%\end{cases}\\
%\text{Weighted:}\quad&\hat{y}_i= 
%\begin{cases}
%    0.5,& \text{if } S(x_i)\geq \gamma_{mb}\\
%    0,              & \text{otherwise}
%\end{cases}
%\end{align}
%The weighted choice is related to learning with positive and unlabeled data \citep{lee2003learning}.




%\subsection{Connection}
%5As follows, we will discuss the connection of our approach to the expectation-maximization (EM) algorithm in latent variable modeling. 

%Our approach bears resembalance to the EM algorithm, where each datapoint is equipped with an unobserved (latent) assignment variable. The algorithm proceeds in two steps: an expectation (E) step, where the latent assignments are inferred, based on the global model parameters, and the maximization (M) step, where the global model parameters are updated, given the inferred assignments. Similarly to the EM algorithm, each datum has an unobserved class assignment value--being an inlier or outlier. Our algorithm decides iteratively on the more likely value of this latent variable (in the case of "radical" LOE), or expresses its ambivalence about it (in the case of "weighted" LOE). 
%
%In the case of density estimation for anomaly detection, one can interpret the loss function as a weighted combination of a density of "normal" samples plus its complement. Our algorithm then proceeds in assigning each datum to either of both cases. The assigned label then, importantly, guides training and influences the density of the normal samples. While normal samples enhance the local density, abnormal samples suppress the density. 
%
%The interpretation of \emph{weighted} latent OE is slightly different. The approach treats the estimated abnormal training samples as unknown and therefore maximizes the information entropy of estimated abnormal training samples. It is still an EM approach in the sense that the inferred labels influence the global model parameters, and in that the algorithm iterates between the two update steps. 

==> Latent Outlier Exposure-ICML2022/pseudo_code.tex <==
\RestyleAlgo{ruled}
\SetKwInput{kwData}{Data}
\SetKwInput{kwModel}{Model}
\SetKwInput{kwInput}{Input}
\begin{algorithm}[t]
\caption{Training process of \gls{loe}}
\label{alg:loe}
\kwInput{Contaminated training set $\mathcal{D}$ ($\alpha_0$ anomaly rate)\\
$\qquad \quad$hyperparamter $\alpha$}
\kwModel{Deep anomaly detector with parameters $\theta$}
\ForEach{Epoch}{
\ForEach{Mini-batch $\mathcal{M}$}{
Calculate the anomaly score $S_i^{train}$ for $\x_i \in \mathcal{M}$\\
Estimate the label $y_i$ given $S_i^{train}$ and $\alpha$ \\ 
Update the parameters $\theta$ by minimizing ${\cal L}(\theta, \y)$ 


%\eIf{Warm-up}
% {Update the parameters $\theta$ by minimizing $\Ln$}
}
}
\end{algorithm}
\vspace{-5pt}

==> Latent Outlier Exposure-ICML2022/related_work.tex <==
\section{Related Work}
\label{sec:related}
We divide our related work into methods for deep anomaly detection, learning on incomplete or contaminated data, and training anomaly detectors on contaminated data. 
\paragraph{Deep anomaly detection.}
Deep learning has played an important role in recent advances in anomaly detection. For example, \citet{ruff2018deep} have improved the anomaly detection accuracy of one-class classification \citep{scholkopf2001estimating} by combining it with a deep feature extractor, both in the unsupervised and the semi-supervised setting \citep{ruff2019deep}. An alternative strategy to combine deep learning with one-class approaches is to train a one-class SVM on pretrained self-supervised features \citep{sohn2020learning}. Indeed, self-supervised learning has influenced deep anomaly detection in a number of ways: The self-supervised criterion for training a deep feature extractor can be used directly to score anomalies \citep{golan2018deep,bergman2020classification}. Using a \gls{mhrot}, \citet{hendrycks2019using} improve self-supervised anomaly detection by solving multiple classification tasks. 
% design \gls{mhrot} a self-supervised anomaly detection method using multiple classification tasks involving handcrafted image transformations while in 
For general data types beyond images, \gls{ntl}~\citep{qiu2021neural,qiu2022raising} learns the transformations for the self-supervision task and achieves solid detection accuracy. \citet{schneider2022detecting} combine \gls{ntl} with representation learning for detecting anomalies within time series.
% are directly learned from data, thereby achieving solid detection accuracy in domains beyond images. 
On tabular data, \gls{icl}~\citep{shenkar2022anomaly} learns feature relations as a self-supervised learning task.
% Another self-supervised approach for anomaly detection on tabular data is \gls{icl} \citep{shenkar2022anomaly}. It employs two encoders to learn the dependence between two complementary subsets of features in the data.
Other classes of deep anomaly detection includes autoencoder variants \citep{principi2017acoustic,zhou2017anomaly,chen2018unsupervised} and density-based models \citep{schlegl2017unsupervised, deecke2018image}.

All these approaches assume a training dataset of ``normal'' data. 
% Their anomaly detection strategy relies on the loss decreasing during training. During test time, the loss is then low for examples that resemble the original training data while being higher for anomalies.
However, in many practical scenarios there will be unlabeled anomalies hidden in the training data. \citet{wang2019effective,huyan2021unsupervised} have shown that anomaly detection accuracy deteriorates when the training set is contaminated. Our work provides a training strategy to deal with contamination. %In this paper we develop a training strategy that can improve existing deep anomaly detectors in the presence of contaminated training data. 

\iffalse
Related work on deep anomaly detection includes deep autoencoder variants \citep{principi2017acoustic,zhou2017anomaly,chen2018unsupervised}, deep generative models \citep{schlegl2017unsupervised, deecke2018image},
\begin{itemize}
    \item One-class classification~\citep{scholkopf2001estimating,ruff2018deep}
        \item Deep Semi-Supervised One-class classification \citep{ruff2019deep}
    \item \citet{sohn2020learning} augments one-class classification with better self-learned data representations.
    \item Using self-supervised learning improves the model robustness to the OOD data~\citep{hendrycks2019using}.
    \item Other self-supervised anomaly detection~\citep{golan2018deep, bergman2020classification}.
    \item \citet{qiu2021neural} extends the self-supervised learning anomaly detection beyond image data.
    \item Auto-encoder based anomaly detection~\citep{zhou2017anomaly}.
    \item TODO: add at least all the models we analyze here.
\end{itemize}


\paragraph{Learning on incomplete/contaminated data.}
\begin{itemize}
    \item The EM algorithm~\citep{dempster1977maximum} iterates between updating a global model and per-datapoint latent variables. K-means clustering~\citep{hartigan1979algorithm} can be considered a special case of EM, although it is usually considered non-probabilistic. Our approach can be considered an EM approach, but we model the assignment labels as discrete and non-probabilistic. 
    \item In semi-supervised setups, \citet{nigam2000text} used a small number of labeled samples and a large number of unlabeled data to classify texts.
    \item \citet{liu2002partially} also investigated text classification with EM algorithm
    \item None of these methods have been used in the context of deep anomaly detection. 
\end{itemize}
\fi

\paragraph{Anomaly Detection on contaminated training data.} 
A common strategy to deal with contaminated training data is to hope that the contamination ratio is low 
and that the anomaly detection method will exercise {\em inlier priority} \citep{wang2019effective}. Throughout our paper, we refer to the strategy of blindly training an anomaly detector as if the training data was clean as ``\textit{Blind}'' training. 
\citet{yoon2021self} have proposed a data refinement strategy that removes potential anomalies from the training data. Their approach, which we refer to as ``{\em Refine}'', employs an ensemble of one-class classifiers to iteratively weed out anomalies and then to continue training on the refined dataset. Similar data refinement strategy are also combined with latent SVDD \citep{gornitz2014learning} or autoencoders for anomaly detection \citep{xia2015learning,beggel2019robust}.
However, these methods fail to exploit the insight of outlier exposure
\citep{hendrycks2018deep} that anomalies provide a valuable training signal.
\citet{zhou2017anomaly} used a robust autoencoder for identifying anomalous training data points, but their approach requires training a new model for identifying anomalies, which is impractical in most setups.  
\citet{hendrycks2018deep} 
propose to artificially contaminate the training data with samples from a related domain which can then be considered anomalies. While outlier exposure assumes labeled anomalies, our work aims at exploiting unlabeled anomalies in the training data.
Notably, \citet{pang2020self} have used an iterative scheme to detect abnormal frames in video clips, and \citet{feng2021mist} extend it to supervised video anomaly detection.
Our work is more general and provides a principled way to improve the training strategy of all approaches mentioned in the paragraph ``deep anomaly detection'' when the training data is likely contaminated.

%The iterative training mechanism is tied to the EM algorithm~\citep{dempster1977maximum} which iterates between updating a global model and per-datapoint latent variables. K-means clustering~\citep{hartigan1979algorithm} can be considered a special case of EM, although it is usually considered non-probabilistic. Our approach can be considered an EM approach, but we model the assignment labels as discrete and non-probabilistic. 
\iffalse
\begin{itemize}
    \item outlier exposure\citep{hendrycks2018deep}. Anomalies are labeled; hence contamination is artificial and provides labeled anomalies.
    \item In unsupervised video anomaly detection, Self-trained Deep Ordinal Regression \citep{pang2020self} learned an anomaly scorer, which is a two-class ordinal regressor, to predict abnormal frames in a video clip. Similar to EM iterations, they repeatedly used the scorer to predict frame labels and re-trained the scorer with the most likely normal and abnormal frames. 
    \item \citet{wang2019effective} show that the performance of anomaly detectors decreases when the training set is contaminated.
    \item \citet{yoon2021self} use an additional ensemble of one-class classifiers to refine the training set in unsupervised anomaly detection. In experiments, we apply this data refinement idea with the ensemble size being 1 as our baseline and we name it \textit{Refine}.
    \item We note that other established anomaly detection techniques on \textit{clean} training data do not prevent their applications on the contaminated training data setup. We thus also apply them to our experiments as another baseline, named \textit{Blind} as we blindly apply the models as if on a clean training dataset.
\end{itemize}
\fi


%\paragraph{Self-training}
%Expectation-Maximization (EM) algorithm~\citep{dempster1977maximum} is designed for modeling with incomplete data. Data with partial labels or missing labels are within this realm. In semi-supervised setups, \citet{nigam2000text} used a small number of labeled samples and a large number of unlabeled data to classify texts. They first initialized a Naive Bayes classifier with labeled data, then improved the classifier with the unlabeled data in EM iterations. Similarly, \citet{liu2002partially} also investigated text classification with EM algorithm, but they focused on separating a specific class of documents from others, given available texts of the desired class and other unlabeled data. The EM algorithm was used to classify the unlabeled data. While this setup is similar to one-class classification~\citep{scholkopf2001estimating,ruff2018deep}, \citet{liu2002partially} further utilized the unlabeled data to improve the model. In unsupervised video anomaly detection, Self-trained Deep Ordinal Regression \citet{pang2020self} learned an anomaly scorer, which is a two-class ordinal regressor, to predict abnormal frames in a video clip. Similar to EM iterations, they repeatedly used the scorer to predict frame labels and re-trained the scorer with the most likely normal and abnormal frames. Our proposed methods improve the above work. Compared to semi-supervised setups, we don't require any labels, which relaxes the constraint; compared to the unsupervised video anomaly detection, our proposed methods are more general as we allow for different loss functions for normal and abnormal data, and proved convergent as a coordinate descent algorithm.
%explicitly connect to EM algorithm.

%\paragraph{Semi-supervised anomaly detection}
%outlier exposure\citep{hendrycks2018deep}

%Deep Semi-Supervised Anomaly Detection \citep{ruff2019deep}
%\paragraph{Unsupervised anomaly detection}
%\citet{wang2019effective} show that the performance of anomaly detectors decreases when the training set is contaminated.
%\citet{yoon2021self} use an additional ensemble of one-class classifiers to refine the training set in unsupervised anomaly detection.

==> Latent Outlier Exposure-ICML2022/tables/image_results.tex <==
\iffalse
\begin{table*}[t!]
%\vspace{-6pt}
	\caption{AUC ($\%$) with standard deviation for anomaly detection on CIFAR-10 and Fashion-MNIST. For all experiments, we set the contamination ratio as $10\%$.}
	\label{tab:image_results}
	\centering
	\vspace{3pt}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{l|ccccc|ccccc}
        \hline
        &\multicolumn{5}{c|}{NTL} &\multicolumn{5}{c}{MHRot}\\
      %  \cline{2-11}
        &Blind& Refine& LOE-H & LOE-S & G-truth & Blind & Refine& LOE-H & LOE-S & G-truth\\
        \hline
        \multirow{2}{*}{CIFAR-10}& 91.7$\pm$0.1 &93.7$\pm$0.1 &94.9$\pm$0.1&95.0$\pm$0.1&99.1\\
        & (-4.0) & (-2.0) & (-0.8) & (-0.7) & (+3.4)\\
        \hline
         \multirow{2}{*}{F-MNIST}&90.4$\pm$0.2 & 92.0$\pm$0.2 & 92.1$\pm$0.5 & 92.5$\pm$0.2 & 98.3\\
         & (-4.3) & (-2.7) & (-2.6) & (-2.2) & (+3.6)\\
        \hline
	\end{tabular}
	}
	\vspace{-5pt}
\end{table*}
\fi
\begin{table}[t!]
%\vspace{-5pt}
	\caption{AUC ($\%$) with standard deviation for anomaly detection on CIFAR-10 and F-MNIST. For all experiments, we set the contamination ratio as $10\%$. \gls{loe} mitigates the performance drop when \gls{ntl} and \gls{mhrot} trained on the contaminated datasets.}
	\label{tab:image_results}
	\small
	\centering
	\vspace{2pt}
%	\resizebox{0.9\linewidth}{!}{
	\begin{tabular}{ll|cc}
        \hline
		     && CIFAR-10   & F-MNIST  \\
		\hline
        \multirow{4}{*}{\rotatebox{90}{NTL}} 
        &Blind &91.3$\pm$0.1 (-4.4) & 85.0$\pm$0.2 (-9.7) \\
        & Refine & 93.5$\pm$0.1 (-2.2) & 89.1$\pm$0.2 (-5.6) \\
        & LOE$_H$ (ours)& \textbf{94.9$\pm$0.2 (-0.8)} & \textbf{92.9$\pm$0.7 (-1.8)} \\
        & LOE$_S$ (ours)& \textbf{94.9$\pm$0.1 (-0.8)} & 92.5$\pm$0.1 (-2.2)\\
%        \cline{2-4}
%        & G-truth & 99.1 (+3.4) & 98.3 (+3.6) \\
        \hline
        \multirow{4}{*}{\rotatebox{90}{MHRot}} 
        &Blind &84.0$\pm$0.5 (-4.2) &88.8$\pm$0.1 (-4.9)\\
        & Refine &84.4$\pm$0.1 (-3.8) &89.6$\pm$0.2 (-4.1)\\
        & LOE$_H$ (ours)&\textbf{86.4$\pm$0.5 (-1.8)} &\textbf{91.4$\pm$0.2 (-2.3)}\\
        & LOE$_S$ (ours)&86.3$\pm$0.2 (-1.9) &91.2$\pm$0.4 (-2.5)\\
%        \cline{2-4}
%        & G-truth &93.5 (+5.3) &98.5 (+4.8)\\
        \hline
	\end{tabular}
%	}
%	\vspace{-5pt}
\end{table}


\begin{table}[t!]
%\vspace{-6pt}
	\caption{AUC ($\%$) with standard deviation of \gls{ntl} for anomaly detection/segmentation on MVTEC. We set the contamination ratio of the training set as $10\%$ and $20\%$.}
	\label{tab:mvtec_results}
	\small
	\centering
	\vspace{2pt}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{l|cc|cc}
        \hline
        &\multicolumn{2}{c|}{Detection} &\multicolumn{2}{c}{Segmentation}\\
       % \cline{2-5}
        & $10\%$ & $20\%$ & $10\%$ & $20\%$\\ 
		\hline
        \multirow{2}{*}{Blind} & 94.2$\pm$0.5 & 89.4$\pm$0.3 & 96.17$\pm$0.08   & 95.09$\pm$0.17  \\
        & (-3.2) & (-8.0) & (-0.78)  & (-1.86)\\
    %    \hline
        \multirow{2}{*}{Refine} & 95.3$\pm$0.5 & 93.2$\pm$0.3 & 96.55$\pm$0.04  & 96.09$\pm$0.06  \\
        & (-2.1) & (-4.2) & (-0.40) & (-0.86)\\
  %      \hline
        LOE$_H$ & \textbf{95.9$\pm$0.9} & 92.9$\pm$0.4 & 95.97$\pm$0.22  & 93.29$\pm$0.21  \\
        (ours)& (-1.5) & (-4.5) & (-0.98) & (-3.66)\\
    %    \hline
        LOE$_S$ & 95.4$\pm$0.5  & \textbf{93.6$\pm$0.3} & \textbf{96.56$\pm$0.04}   & \textbf{96.11$\pm$0.05}  \\
        (ours)& (-2.0) & (-3.8) & (-0.39) & (-0.84)\\
        \hline
%         G-truth\\
	\end{tabular}
	}
	%\vspace{-5pt}
\end{table}



==> Latent Outlier Exposure-ICML2022/tables/negative_losses.tex <==
\begin{table}[ht]
%\vspace{-6pt}
	\caption{$\La$ for various anomaly detectors.}
	\label{tab:anomaly loss}
	\centering
	\vspace{3pt}
%	\resizebox{\linewidth}{!}{
	\begin{tabular}{l|c}
        \hline
        & $\La$\\
        \hline
         \vspace{5pt}       
        MHRot& 
   $ \sum_{c=1}^{|\mathcal{T}|}\sum_{l=1}^3 \text{CE}(\mathcal{U}, p_l(\cdot \mid f,T_c(\x)))$\\
        \vspace{5pt}
        NTL& $-\sum_{k=1}^K \log (1-p_k(x\mid f,\mathcal{T}))$\\
        \vspace{5pt}
        ICL& $-\sum_{k=1}^K \log (1-p_k(x\mid f,g,\mathcal{T}))$\\
        \vspace{5pt}
        DSVDD & $1/||f(x)-c||^2 $\\
        \hline
	\end{tabular}
%	}
	\vspace{-5pt}
\end{table}

==> Latent Outlier Exposure-ICML2022/tables/small_tabular_results.tex <==
\begin{table*}[t!]
%\vspace{-6pt}
	\caption{F1-score ($\%$) for anomaly detection on $30$ tabular datasets studied in \citep{shenkar2022anomaly}. We set $\alpha_0=\alpha=10\%$ in all experiments. 
	\gls{loe} (proposed) outperforms the ``Blind'' and ``Refine'' consistently. (See \cref{tab:tabular_f1,tab:tabular_auc} for more details, including AUCs.)}
	\label{tab:tabular_small}
	\small
	\centering
	\vspace{2pt}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{l|cccc|cccc}
        \hline
        &\multicolumn{4}{c|}{NTL}&\multicolumn{4}{c}{ICL} \\
      %  \cline{2-11}
        &Blind& Refine& LOE$_H$ (ours)& LOE$_S$ (ours)&Blind& Refine& LOE$_H$ (ours)& LOE$_S$ (ours)\\
        \hline
abalone	& 37.9$\pm$13.4& 55.2$\pm$15.9& 42.8$\pm$26.9& \textbf{59.3$\pm$12.0}& 50.9$\pm$1.5& \textbf{54.3$\pm$2.9}& 53.4$\pm$5.2& 51.7$\pm$2.4\\ 
annthyroid	& 29.7$\pm$3.5& 42.7$\pm$7.1& 47.7$\pm$11.4& \textbf{50.3$\pm$4.5}& 29.1$\pm$2.2& 38.5$\pm$2.1& \textbf{48.7$\pm$7.6}& 43.0$\pm$8.8\\ 
arrhythmia	& 57.6$\pm$2.5& 59.1$\pm$2.1& 62.1$\pm$2.8& \textbf{62.7$\pm$3.3}& 53.9$\pm$0.7& 60.9$\pm$2.2& 62.4$\pm$1.8& \textbf{63.6$\pm$2.1}\\ 
breastw	& 84.0$\pm$1.8& 93.1$\pm$0.9& \textbf{95.6$\pm$0.4}& 95.3$\pm$0.4& 92.6$\pm$1.1& 93.4$\pm$1.0& \textbf{96.0$\pm$0.6}& 95.7$\pm$0.6\\ 
cardio	& 21.8$\pm$4.9& 45.2$\pm$7.9& \textbf{73.0$\pm$7.9}& 57.8$\pm$5.5& 50.2$\pm$4.5& 56.2$\pm$3.4& \textbf{71.1$\pm$3.2}& 62.2$\pm$2.7\\ 
ecoli	& 0.0$\pm$0.0& 88.9$\pm$14.1& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& 17.8$\pm$15.1& 46.7$\pm$25.7& \textbf{75.6$\pm$4.4}& \textbf{75.6$\pm$4.4}\\ 
forest cover	& 20.4$\pm$4.0& 56.2$\pm$4.9& 61.1$\pm$34.9& \textbf{67.6$\pm$30.6}& 9.2$\pm$4.5& 8.0$\pm$3.6& 6.8$\pm$3.6& \textbf{11.1$\pm$2.1}\\ 
glass	& 11.1$\pm$7.0& 15.6$\pm$5.4& 17.8$\pm$5.4& \textbf{20.0$\pm$8.3}& 8.9$\pm$4.4& \textbf{11.1$\pm$0.0}& \textbf{11.1$\pm$7.0}& 8.9$\pm$8.3\\ 
ionosphere	& 89.0$\pm$1.5& 91.0$\pm$2.0& 91.0$\pm$1.7& \textbf{91.3$\pm$2.2}& 86.5$\pm$1.1& 85.9$\pm$2.3& 85.7$\pm$2.8& \textbf{88.6$\pm$0.6}\\ 
kdd	& 95.9$\pm$0.0& 96.0$\pm$1.1& 98.1$\pm$0.4& \textbf{98.4$\pm$0.1}& 99.3$\pm$0.1& 99.4$\pm$0.1& \textbf{99.5$\pm$0.0}& 99.4$\pm$0.0\\ 
kddrev	& 98.4$\pm$0.1& 98.4$\pm$0.2& 89.1$\pm$1.7& \textbf{98.6$\pm$0.0}& 97.9$\pm$0.5& 98.4$\pm$0.4& \textbf{98.8$\pm$0.1}& 98.2$\pm$0.4\\ 
letter	& 36.4$\pm$3.6& 44.4$\pm$3.1& 25.4$\pm$10.0& \textbf{45.6$\pm$10.6}& 43.0$\pm$2.5& 51.2$\pm$3.7& \textbf{54.4$\pm$5.6}& 47.2$\pm$4.9\\ 
lympho	& 53.3$\pm$12.5& 60.0$\pm$8.2& 60.0$\pm$13.3& \textbf{73.3$\pm$22.6}& 43.3$\pm$8.2& 60.0$\pm$8.2& 80.0$\pm$12.5& \textbf{83.3$\pm$10.5}\\ 
mammogra.	& 5.5$\pm$2.8& 2.6$\pm$1.7& 3.3$\pm$1.6& \textbf{13.5$\pm$3.8}& 8.8$\pm$1.9& 11.4$\pm$1.9& 34.0$\pm$20.2& \textbf{42.8$\pm$17.6}\\ 
mnist tabular	& 78.6$\pm$0.5& \textbf{80.3$\pm$1.1}& 71.8$\pm$1.8& 76.3$\pm$2.1& 72.1$\pm$1.0& 80.7$\pm$0.7& \textbf{86.0$\pm$0.4}& 79.2$\pm$0.9\\ 
mulcross	& 45.5$\pm$9.6& \textbf{58.2$\pm$3.5}& \textbf{58.2$\pm$6.2}& 50.1$\pm$8.9& 70.4$\pm$13.4& 94.4$\pm$6.3& \textbf{100$\pm$0.0}& 99.9$\pm$0.1\\ 
musk	& 21.0$\pm$3.3& 98.8$\pm$0.4& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& 6.2$\pm$3.0& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}\\ 
optdigits	& 0.2$\pm$0.3& 1.5$\pm$0.3& 41.7$\pm$45.9& \textbf{59.1$\pm$48.2}& 0.8$\pm$0.5& \textbf{1.3$\pm$1.1}& 1.2$\pm$1.0& 0.9$\pm$0.5\\ 
pendigits	& 5.0$\pm$2.5& 32.6$\pm$10.0& 79.4$\pm$4.7& \textbf{81.9$\pm$4.3}& 10.3$\pm$4.6& 30.1$\pm$8.5& 80.3$\pm$6.1& \textbf{88.6$\pm$2.2}\\ 
pima	& 60.3$\pm$2.6& 61.0$\pm$1.9& \textbf{61.3$\pm$2.4}& 61.0$\pm$0.9& 58.1$\pm$2.9& 59.3$\pm$1.4& \textbf{63.0$\pm$1.0}& 60.1$\pm$1.4\\ 
satellite	& 73.6$\pm$0.4& 74.1$\pm$0.3& \textbf{74.8$\pm$0.4}& 74.7$\pm$0.1& 72.7$\pm$1.3& 72.7$\pm$0.6& \textbf{73.6$\pm$0.2}& 73.2$\pm$0.6\\ 
satimage	& 26.8$\pm$1.5& 86.8$\pm$4.0& 90.7$\pm$1.1& \textbf{91.0$\pm$0.7}& 7.3$\pm$0.6& 85.1$\pm$1.4& 91.3$\pm$1.1& \textbf{91.5$\pm$0.9}\\ 
seismic	& 11.9$\pm$1.8& 11.5$\pm$1.0& \textbf{18.1$\pm$0.7}& 17.1$\pm$0.6& 14.9$\pm$1.4& 17.3$\pm$2.1& 23.6$\pm$2.8& \textbf{24.2$\pm$1.4}\\ 
shuttle	& 97.0$\pm$0.3& 97.0$\pm$0.2& \textbf{97.1$\pm$0.2}& 97.0$\pm$0.2& 96.6$\pm$0.2& 96.7$\pm$0.1& 96.9$\pm$0.1& \textbf{97.0$\pm$0.2}\\ 
speech	& 6.9$\pm$1.2& 8.2$\pm$2.1& 43.3$\pm$5.6& \textbf{50.8$\pm$2.5}& 0.3$\pm$0.7& 1.6$\pm$1.0& \textbf{2.0$\pm$0.7}& 0.7$\pm$0.8\\ 
thyroid	& 43.4$\pm$5.5& 55.1$\pm$4.2& \textbf{82.4$\pm$2.7}& \textbf{82.4$\pm$2.3}& 45.8$\pm$7.3& 71.6$\pm$2.4& \textbf{83.2$\pm$2.9}& 80.9$\pm$2.5\\ 
vertebral	& 22.0$\pm$4.5& 21.3$\pm$4.5& 22.7$\pm$11.0& \textbf{25.3$\pm$4.0}& 8.9$\pm$3.1& 8.9$\pm$4.2& 7.8$\pm$4.2& \textbf{10.0$\pm$2.7}\\ 
vowels	& 36.0$\pm$1.8& 50.4$\pm$8.8& \textbf{62.8$\pm$9.5}& 48.4$\pm$6.6& 42.1$\pm$9.0& 60.4$\pm$7.9& \textbf{81.6$\pm$2.9}& 74.4$\pm$8.0\\ 
wbc	& 25.7$\pm$12.3& 45.7$\pm$15.5& \textbf{76.2$\pm$6.0}& 69.5$\pm$3.8& 50.5$\pm$5.7& 50.5$\pm$2.3& \textbf{61.0$\pm$4.7}& \textbf{61.0$\pm$1.9}\\ 
wine	& 24.0$\pm$18.5& 66.0$\pm$12.0& 90.0$\pm$0.0& \textbf{92.0$\pm$4.0}& 4.0$\pm$4.9& 10.0$\pm$8.9& 98.0$\pm$4.0& \textbf{100$\pm$0.0}\\ 
\hline
	\end{tabular}
	}
%	\vspace{-5pt}
\end{table*}

==> Latent Outlier Exposure-ICML2022/tables/tabular_results.tex <==
\begin{table*}[t!]
%\vspace{-6pt}
	\caption{F1-score ($\%$) with standard deviation for anomaly detection on 30 tabular datasets which are from the empirical study of \citet{shenkar2022anomaly}. For all experiments, we set the contamination ratio of the training set as $10\%$. The number in the brackets is the average performance difference from the model trained on clean data. 
	\gls{loe} outperforms the ``Blind'' and ``Refine'' baselines.}
	\label{tab:tabular_f1}
	\small
	\centering
	\vspace{3pt}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{lcccc|cccc}
        \hline
        &\multicolumn{4}{c|}{NTL}&\multicolumn{4}{c}{ICL} \\
      %  \cline{2-11}
        &Blind& Refine& LOE$_H$ (ours)& LOE$_S$ (ours)&Blind& Refine& LOE$_H$ (ours)& LOE$_S$ (ours)\\
        \hline
\multirow{2}{*}{abalone}	& 37.9$\pm$13.4& 55.2$\pm$15.9& 42.8$\pm$26.9& \textbf{59.3$\pm$12.0}& 50.9$\pm$1.5& \textbf{54.3$\pm$2.9}& 53.4$\pm$5.2& 51.7$\pm$2.4\\ 
&(-25.3)&(-8.0)&(-20.4)& \textbf{(-3.9)}&(-11.2)& \textbf{(-7.8)}&(-8.7)&(-10.4)\\ 
\multirow{2}{*}{annthyroid}	& 29.7$\pm$3.5& 42.7$\pm$7.1& 47.7$\pm$11.4& \textbf{50.3$\pm$4.5}& 29.1$\pm$2.2& 38.5$\pm$2.1& \textbf{48.7$\pm$7.6}& 43.0$\pm$8.8\\ 
&(-21.6)&(-8.6)&(-3.6)& \textbf{(-1.0)}&(-12.0)&(-2.6)& \textbf{(+7.6)}&(+1.9)\\ 
\multirow{2}{*}{arrhythmia}	& 57.6$\pm$2.5& 59.1$\pm$2.1& 62.1$\pm$2.8& \textbf{62.7$\pm$3.3}& 53.9$\pm$0.7& 60.9$\pm$2.2& 62.4$\pm$1.8& \textbf{63.6$\pm$2.1}\\ 
&(-3.0)&(-1.5)&(+1.5)& \textbf{(+2.1)}&(-7.6)&(-0.6)&(+0.9)& \textbf{(+2.1)}\\ 
\multirow{2}{*}{breastw}	& 84.0$\pm$1.8& 93.1$\pm$0.9& \textbf{95.6$\pm$0.4}& 95.3$\pm$0.4& 92.6$\pm$1.1& 93.4$\pm$1.0& \textbf{96.0$\pm$0.6}& 95.7$\pm$0.6\\ 
&(-8.4)&(+0.7)& \textbf{(+3.2)}&(+2.9)&(-2.4)&(-1.6)& \textbf{(+1.0)}&(+0.7)\\ 
\multirow{2}{*}{cardio}	& 21.8$\pm$4.9& 45.2$\pm$7.9& \textbf{73.0$\pm$7.9}& 57.8$\pm$5.5& 50.2$\pm$4.5& 56.2$\pm$3.4& \textbf{71.1$\pm$3.2}& 62.2$\pm$2.7\\ 
&(-35.0)&(-11.6)& \textbf{(+16.2)}&(+1.0)&(-19.5)&(-13.5)& \textbf{(+1.4)}&(-7.5)\\ 
\multirow{2}{*}{ecoli}	& 0.0$\pm$0.0& 88.9$\pm$14.1& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& 17.8$\pm$15.1& 46.7$\pm$25.7& \textbf{75.6$\pm$4.4}& \textbf{75.6$\pm$4.4}\\ 
&(-95.6)&(-6.7)& \textbf{(+4.4)}&\textbf{(+4.4)}&(-55.5)&(-26.6)& \textbf{(+2.3)}&\textbf{(+2.3)}\\ 
\multirow{2}{*}{forest cover}	& 20.4$\pm$4.0& 56.2$\pm$4.9& 61.1$\pm$34.9& \textbf{67.6$\pm$30.6}& 9.2$\pm$4.5& 8.0$\pm$3.6& 6.8$\pm$3.6& \textbf{11.1$\pm$2.1}\\ 
&(-44.2)&(-8.4)&(-3.5)& \textbf{(+3.0)}&(-37.8)&(-39.0)&(-40.2)& \textbf{(-35.9)}\\ 
\multirow{2}{*}{glass}	& 11.1$\pm$7.0& 15.6$\pm$5.4& 17.8$\pm$5.4& \textbf{20.0$\pm$8.3}& 8.9$\pm$4.4& \textbf{11.1$\pm$0.0}& 11.1$\pm$7.0& 8.9$\pm$8.3\\ 
&(-6.7)&(-2.2)&(+0.0)& \textbf{(+2.2)}&(-13.3)& \textbf{(-11.1)}&(-11.1)&(-13.3)\\ 
\multirow{2}{*}{ionosphere}	& 89.0$\pm$1.5& 91.0$\pm$2.0& 91.0$\pm$1.7& \textbf{91.3$\pm$2.2}& 86.5$\pm$1.1& 85.9$\pm$2.3& 85.7$\pm$2.8& \textbf{88.6$\pm$0.6}\\ 
&(-3.5)&(-1.5)&(-1.5)& \textbf{(-1.2)}&(-5.7)&(-6.3)&(-6.5)& \textbf{(-3.6)}\\ 
\multirow{2}{*}{kdd}	& 95.9$\pm$0.0& 96.0$\pm$1.1& 98.1$\pm$0.4& \textbf{98.4$\pm$0.1}& 99.3$\pm$0.1& 99.4$\pm$0.1& \textbf{99.5$\pm$0.0}& 99.4$\pm$0.0\\ 
&(-2.4)&(-2.3)&(-0.2)& \textbf{(+0.1)}&(-0.1)&(+0.0)& \textbf{(+0.1)}&(+0.0)\\ 
\multirow{2}{*}{kddrev}	& 98.4$\pm$0.1& 98.4$\pm$0.2& 89.1$\pm$1.7& \textbf{98.6$\pm$0.0}& 97.9$\pm$0.5& 98.4$\pm$0.4& \textbf{98.8$\pm$0.1}& 98.2$\pm$0.4\\ 
&(+0.2)&(+0.2)&(-9.1)& \textbf{(+0.4)}&(-0.9)&(-0.4)& \textbf{(+0.0)}&(-0.6)\\ 
\multirow{2}{*}{letter}	& 36.4$\pm$3.6& 44.4$\pm$3.1& 25.4$\pm$10.0& \textbf{45.6$\pm$10.6}& 43.0$\pm$2.5& 51.2$\pm$3.7& \textbf{54.4$\pm$5.6}& 47.2$\pm$4.9\\ 
&(-11.0)&(-3.0)&(-22.0)& \textbf{(-1.8)}&(-15.5)&(-7.3)& \textbf{(-4.1)}&(-11.3)\\ 
\multirow{2}{*}{lympho}	& 53.3$\pm$12.5& 60.0$\pm$8.2& 60.0$\pm$13.3& \textbf{73.3$\pm$22.6}& 43.3$\pm$8.2& 60.0$\pm$8.2& 80.0$\pm$12.5& \textbf{83.3$\pm$10.5}\\ 
&(-20.0)&(-13.3)&(-13.3)& \textbf{(+0.0)}&(-40.0)&(-23.3)&(-3.3)& \textbf{(+0.0)}\\ 
\multirow{2}{*}{mammogra.}	& 5.5$\pm$2.8& 2.6$\pm$1.7& 3.3$\pm$1.6& \textbf{13.5$\pm$3.8}& 8.8$\pm$1.9& 11.4$\pm$1.9& 34.0$\pm$20.2& \textbf{42.8$\pm$17.6}\\ 
&(-21.3)&(-24.2)&(-23.5)& \textbf{(-13.3)}&(-14.0)&(-11.4)&(+11.2)& \textbf{(+20.0)}\\ 
\multirow{2}{*}{mnist tabular}	& 78.6$\pm$0.5& \textbf{80.3$\pm$1.1}& 71.8$\pm$1.8& 76.3$\pm$2.1& 72.1$\pm$1.0& 80.7$\pm$0.7& \textbf{86.0$\pm$0.4}& 79.2$\pm$0.9\\ 
&(-6.6)& \textbf{(-4.9)}&(-13.4)&(-8.9)&(-10.5)&(-1.9)& \textbf{(+3.4)}&(-3.4)\\ 
\multirow{2}{*}{mulcross}	& 45.5$\pm$9.6& \textbf{58.2$\pm$3.5}& \textbf{58.2$\pm$6.2}& 50.1$\pm$8.9& 70.4$\pm$13.4& 94.4$\pm$6.3& \textbf{100$\pm$0.0}& 99.9$\pm$0.1\\ 
&(-50.5)& \textbf{(-37.8)}&\textbf{(-37.8)}&(-45.9)&(-29.6)&(-5.6)& \textbf{(+0.0)}&(-0.1)\\ 
\multirow{2}{*}{musk}	& 21.0$\pm$3.3& 98.8$\pm$0.4& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& 6.2$\pm$3.0& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}\\ 
&(-79.0)&(-1.2)& \textbf{(+0.0)}&\textbf{(+0.0)}&(-93.8)& \textbf{(+0.0)}&\textbf{(+0.0)}&\textbf{(+0.0)}\\ 
\multirow{2}{*}{optdigits}	& 0.2$\pm$0.3& 1.5$\pm$0.3& 41.7$\pm$45.9& \textbf{59.1$\pm$48.2}& 0.8$\pm$0.5& \textbf{1.3$\pm$1.1}& 1.2$\pm$1.0& 0.9$\pm$0.5\\ 
&(-24.7)&(-23.4)&(+16.8)& \textbf{(+34.2)}&(-62.4)& \textbf{(-61.9)}&(-62.0)&(-62.3)\\ 
\multirow{2}{*}{pendigits}	& 5.0$\pm$2.5& 32.6$\pm$10.0& 79.4$\pm$4.7& \textbf{81.9$\pm$4.3}& 10.3$\pm$4.6& 30.1$\pm$8.5& 80.3$\pm$6.1& \textbf{88.6$\pm$2.2}\\ 
&(-56.3)&(-28.7)&(+18.1)& \textbf{(+20.6)}&(-67.9)&(-48.1)&(+2.1)& \textbf{(+10.4)}\\ 
\multirow{2}{*}{pima}	& 60.3$\pm$2.6& 61.0$\pm$1.9& \textbf{61.3$\pm$2.4}& 61.0$\pm$0.9& 58.1$\pm$2.9& 59.3$\pm$1.4& \textbf{63.0$\pm$1.0}& 60.1$\pm$1.4\\ 
&(-1.2)&(-0.5)& \textbf{(-0.2)}&(-0.5)&(-2.2)&(-1.0)& \textbf{(+2.7)}&(-0.2)\\ 
\multirow{2}{*}{satellite}	& 73.6$\pm$0.4& 74.1$\pm$0.3& \textbf{74.8$\pm$0.4}& 74.7$\pm$0.1& 72.7$\pm$1.3& 72.7$\pm$0.6& \textbf{73.6$\pm$0.2}& 73.2$\pm$0.6\\ 
&(-1.0)&(-0.5)& \textbf{(+0.2)}&(+0.1)&(-2.1)&(-2.1)& \textbf{(-1.2)}&(-1.6)\\ 
\multirow{2}{*}{satimage}	& 26.8$\pm$1.5& 86.8$\pm$4.0& 90.7$\pm$1.1& \textbf{91.0$\pm$0.7}& 7.3$\pm$0.6& 85.1$\pm$1.4& 91.3$\pm$1.1& \textbf{91.5$\pm$0.9}\\ 
&(-65.2)&(-5.2)&(-1.3)& \textbf{(-1.0)}&(-82.0)&(-4.2)&(+2.0)& \textbf{(+2.2)}\\ 
\multirow{2}{*}{seismic}	& 11.9$\pm$1.8& 11.5$\pm$1.0& \textbf{18.1$\pm$0.7}& 17.1$\pm$0.6& 14.9$\pm$1.4& 17.3$\pm$2.1& 23.6$\pm$2.8& \textbf{24.2$\pm$1.4}\\ 
&(-0.6)&(-1.0)& \textbf{(+5.6)}&(+4.6)&(-3.0)&(-0.6)&(+5.7)& \textbf{(+6.3)}\\ 
\multirow{2}{*}{shuttle}	& 97.0$\pm$0.3& 97.0$\pm$0.2& \textbf{97.1$\pm$0.2}& 97.0$\pm$0.2& 96.6$\pm$0.2& 96.7$\pm$0.1& 96.9$\pm$0.1& \textbf{97.0$\pm$0.2}\\ 
&(+0.3)&(+0.3)& \textbf{(+0.4)}&(+0.3)&(-0.4)&(-0.3)&(-0.1)& \textbf{(+0.0)}\\ 
\multirow{2}{*}{speech}	& 6.9$\pm$1.2& 8.2$\pm$2.1& 43.3$\pm$5.6& \textbf{50.8$\pm$2.5}& 0.3$\pm$0.7& 1.6$\pm$1.0& \textbf{2.0$\pm$0.7}& 0.7$\pm$0.8\\ 
&(-2.6)&(-1.3)&(+33.8)& \textbf{(+41.3)}&(-4.1)&(-2.8)& \textbf{(-2.4)}&(-3.7)\\ 
\multirow{2}{*}{thyroid}	& 43.4$\pm$5.5& 55.1$\pm$4.2& \textbf{82.4$\pm$2.7}& \textbf{82.4$\pm$2.3}& 45.8$\pm$7.3& 71.6$\pm$2.4& \textbf{83.2$\pm$2.9}& 80.9$\pm$2.5\\ 
&(-34.4)&(-22.7)& \textbf{(+4.6)}&\textbf{(+4.6)}&(-31.4)&(-5.6)& \textbf{(+6.0)}&(+3.7)\\ 
\multirow{2}{*}{vertebral}	& 22.0$\pm$4.5& 21.3$\pm$4.5& 22.7$\pm$11.0& \textbf{25.3$\pm$4.0}& 8.9$\pm$3.1& 8.9$\pm$4.2& 7.8$\pm$4.2& \textbf{10.0$\pm$2.7}\\ 
&(-8.7)&(-9.4)&(-8.0)& \textbf{(-5.4)}&(-7.8)&(-7.8)&(-8.9)& \textbf{(-6.7)}\\ 
\multirow{2}{*}{vowels}	& 36.0$\pm$1.8& 50.4$\pm$8.8& \textbf{62.8$\pm$9.5}& 48.4$\pm$6.6& 42.1$\pm$9.0& 60.4$\pm$7.9& \textbf{81.6$\pm$2.9}& 74.4$\pm$8.0\\ 
&(-40.7)&(-26.3)& \textbf{(-13.9)}&(-28.3)&(-37.5)&(-19.2)& \textbf{(+2.0)}&(-5.2)\\ 
\multirow{2}{*}{wbc}	& 25.7$\pm$12.3& 45.7$\pm$15.5& \textbf{76.2$\pm$6.0}& 69.5$\pm$3.8& 50.5$\pm$5.7& 50.5$\pm$2.3& \textbf{61.0$\pm$4.7}& \textbf{61.0$\pm$1.9}\\ 
&(-39.1)&(-19.1)& \textbf{(+11.4)}&(+4.7)&(-8.2)&(-8.2)& \textbf{(+2.3)}&\textbf{(+2.3)}\\ 
\multirow{2}{*}{wine}	& 24.0$\pm$18.5& 66.0$\pm$12.0& 90.0$\pm$0.0& \textbf{92.0$\pm$4.0}& 4.0$\pm$4.9& 10.0$\pm$8.9& 98.0$\pm$4.0& \textbf{100$\pm$0.0}\\ 
&(-68.0)&(-26.0)&(-2.0)& \textbf{(+0.0)}&(-86.0)&(-80.0)&(+8.0)& \textbf{(+10.0)}\\ 
\hline
	\end{tabular}
	}
	%\vspace{-5pt}
\end{table*}

\begin{table*}[t!]
%\vspace{-6pt}
	\caption{AUC ($\%$) with standard deviation for anomaly detection on 30 tabular datasets which are from the empirical study of \citet{shenkar2022anomaly}. For all experiments, we set the contamination ratio of the training set as $10\%$. The number in the brackets is the average performance difference from the model trained on clean data. 
	\gls{loe} outperforms the ``Blind'' and ``Refine'' baselines.}
	\label{tab:tabular_auc}
	\small
	\centering
	\vspace{3pt}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{lcccc|cccc}
        \hline
        &\multicolumn{4}{c|}{NTL}&\multicolumn{4}{c}{ICL} \\
      %  \cline{2-11}
        &Blind& Refine& LOE$_H$ (ours)& LOE$_S$ (ours)&Blind& Refine& LOE$_H$ (ours)& LOE$_S$ (ours)\\
        \hline
\multirow{2}{*}{abalone}	& 91.4$\pm$1.7& 93.3$\pm$1.7& 93.4$\pm$1.0& \textbf{94.6$\pm$1.4}& 83.1$\pm$1.5& 91.2$\pm$0.8& 93.5$\pm$1.0& \textbf{93.6$\pm$0.8}\\ 
&(-2.4)&(-0.5)&(-0.4)& \textbf{(+0.8)}&(-10.1)&(-2.0)&(+0.3)& \textbf{(+0.4)}\\ 
\multirow{2}{*}{annthyroid}	& 66.1$\pm$2.8& 78.2$\pm$6.6& 83.9$\pm$7.0& \textbf{85.9$\pm$4.8}& 65.5$\pm$2.3& 73.1$\pm$2.5& \textbf{82.4$\pm$5.6}& 76.7$\pm$6.8\\ 
&(-19.1)&(-7.0)&(-1.3)& \textbf{(+0.7)}&(-8.7)&(-1.1)& \textbf{(+8.2)}&(+2.5)\\ 
\multirow{2}{*}{arrhythmia}	& 80.5$\pm$1.1& 82.5$\pm$0.8& 82.7$\pm$1.8& \textbf{84.8$\pm$1.7}& 75.5$\pm$0.3& 77.1$\pm$0.7& \textbf{79.2$\pm$0.2}& 78.4$\pm$0.8\\ 
&(-0.7)&(+1.3)&(+1.5)& \textbf{(+3.6)}&(-2.3)&(-0.7)& \textbf{(+1.4)}&(+0.6)\\ 
\multirow{2}{*}{breastw}	& 89.5$\pm$2.1& 96.1$\pm$0.8& \textbf{99.0$\pm$0.3}& 98.2$\pm$0.5& 97.1$\pm$0.8& 97.4$\pm$0.8& 98.7$\pm$0.3& \textbf{98.8$\pm$0.4}\\ 
&(-6.8)&(-0.2)& \textbf{(+2.7)}&(+1.9)&(-1.0)&(-0.7)&(+0.6)& \textbf{(+0.7)}\\ 
\multirow{2}{*}{cardio}	& 63.5$\pm$3.8& 76.9$\pm$3.8& \textbf{92.6$\pm$3.7}& 85.3$\pm$4.2& 80.0$\pm$1.4& 83.3$\pm$0.9& \textbf{91.1$\pm$1.9}& 87.5$\pm$2.1\\ 
&(-19.7)&(-6.3)& \textbf{(+9.4)}&(+2.1)&(-10.0)&(-6.7)& \textbf{(+1.1)}&(-2.5)\\ 
\multirow{2}{*}{ecoli}	& 74.9$\pm$8.2& 99.6$\pm$0.5& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& 80.4$\pm$4.2& 85.8$\pm$1.5& 88.5$\pm$1.8& \textbf{89.1$\pm$0.8}\\ 
&(-24.9)&(-0.2)& \textbf{(+0.2)}&\textbf{(+0.2)}&(-8.8)&(-3.4)&(-0.7)& \textbf{(-0.1)}\\ 
\multirow{2}{*}{forest cover}	& 91.2$\pm$2.2& \textbf{98.6$\pm$0.7}& 97.7$\pm$2.7& \textbf{98.6$\pm$2.1}& 73.0$\pm$11.7& 77.8$\pm$6.7& 78.9$\pm$3.2& \textbf{81.7$\pm$2.7}\\ 
&(-7.4)& \textbf{(+0.0)}&(-0.9)&\textbf{(+0.0)}&(-22.3)&(-17.5)&(-16.4)& \textbf{(-13.6)}\\ 
\multirow{2}{*}{glass}	& 75.1$\pm$4.0& 76.6$\pm$3.3& \textbf{77.8$\pm$4.8}& 77.1$\pm$4.6& 54.7$\pm$11.4& 66.6$\pm$5.7& 65.4$\pm$12.0& \textbf{71.5$\pm$9.2}\\ 
&(+2.6)&(+4.1)& \textbf{(+5.3)}&(+4.6)&(-25.9)&(-14.0)&(-15.2)& \textbf{(-9.1)}\\ 
\multirow{2}{*}{ionosphere}	& 95.6$\pm$0.8& \textbf{96.8$\pm$0.8}& 96.1$\pm$1.0& \textbf{96.8$\pm$0.9}& 92.6$\pm$1.1& 93.3$\pm$1.3& 88.7$\pm$3.3& \textbf{93.4$\pm$1.0}\\ 
&(-2.3)& \textbf{(-1.1)}&(-1.8)&\textbf{(-1.1)}&(-4.9)&(-4.2)&(-8.8)& \textbf{(-4.1)}\\ 
\multirow{2}{*}{kdd}	& \textbf{99.7$\pm$0.0}& 99.4$\pm$0.2& \textbf{99.7$\pm$0.0}& \textbf{99.7$\pm$0.0}& \textbf{99.9$\pm$0.0}& \textbf{99.9$\pm$0.0}& \textbf{99.9$\pm$0.0}& \textbf{99.9$\pm$0.0}\\ 
& \textbf{(-0.2)}&(-0.5)&\textbf{(-0.2)}&\textbf{(-0.2)}& \textbf{(+0.0)}&\textbf{(+0.0)}&\textbf{(+0.0)}&\textbf{(+0.0)}\\ 
\multirow{2}{*}{kddrev}	& \textbf{99.5$\pm$0.1}& 99.4$\pm$0.1& 96.1$\pm$0.9& \textbf{99.5$\pm$0.1}& 99.5$\pm$0.2& 99.7$\pm$0.1& \textbf{99.8$\pm$0.0}& 99.6$\pm$0.1\\ 
& \textbf{(+0.0)}&(-0.1)&(-3.4)&\textbf{(+0.0)}&(-0.3)&(-0.1)& \textbf{(+0.0)}&(-0.2)\\ 
\multirow{2}{*}{letter}	& 79.8$\pm$0.5& 83.5$\pm$0.8& 76.2$\pm$6.0& \textbf{84.3$\pm$4.8}& 82.3$\pm$2.9& 84.1$\pm$2.0& \textbf{86.2$\pm$2.8}& 83.7$\pm$2.0\\ 
&(-5.0)&(-1.3)&(-8.6)& \textbf{(-0.5)}&(-5.4)&(-3.6)& \textbf{(-1.5)}&(-4.0)\\ 
\multirow{2}{*}{lympho}	& 90.8$\pm$6.7& 93.7$\pm$3.2& 96.6$\pm$1.7& \textbf{98.1$\pm$2.2}& 94.1$\pm$2.0& 96.1$\pm$1.0& \textbf{98.9$\pm$1.0}& \textbf{98.9$\pm$1.1}\\ 
&(-6.3)&(-3.4)&(-0.5)& \textbf{(+1.0)}&(-5.3)&(-3.3)& \textbf{(-0.5)}&\textbf{(-0.5)}\\ 
\multirow{2}{*}{mammogra.}	& 68.7$\pm$6.2& 67.8$\pm$2.0& 69.2$\pm$3.8& \textbf{78.5$\pm$3.2}& 64.2$\pm$4.3& 69.7$\pm$4.7& 80.0$\pm$7.7& \textbf{84.0$\pm$4.3}\\ 
&(-13.8)&(-14.7)&(-13.3)& \textbf{(-4.0)}&(-14.8)&(-9.3)&(+1.0)& \textbf{(+5.0)}\\ 
\multirow{2}{*}{mnist tabular}	& 96.1$\pm$0.2& \textbf{96.7$\pm$0.4}& 94.7$\pm$0.5& 96.1$\pm$0.4& 94.1$\pm$0.4& 96.4$\pm$0.3& \textbf{97.9$\pm$0.1}& 96.3$\pm$0.2\\ 
&(-1.9)& \textbf{(-1.3)}&(-3.3)&(-1.9)&(-3.1)&(-0.8)& \textbf{(+0.7)}&(-0.9)\\ 
\multirow{2}{*}{mulcross}	& 81.7$\pm$7.5& \textbf{91.2$\pm$1.4}& 90.8$\pm$4.5& 82.6$\pm$10.5& 93.7$\pm$4.4& 99.4$\pm$0.7& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}\\ 
&(-17.9)& \textbf{(-8.4)}&(-8.8)&(-17.0)&(-6.3)&(-0.6)& \textbf{(+0.0)}&\textbf{(+0.0)}\\ 
\multirow{2}{*}{musk}	& 76.2$\pm$2.3& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& 78.8$\pm$2.9& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}& \textbf{100$\pm$0.0}\\ 
&(-23.8)& \textbf{(+0.0)}&\textbf{(+0.0)}&\textbf{(+0.0)}&(-21.2)& \textbf{(+0.0)}&\textbf{(+0.0)}&\textbf{(+0.0)}\\ 
\multirow{2}{*}{optdigits}	& 31.0$\pm$3.7& 38.7$\pm$3.8& 70.9$\pm$27.8& \textbf{72.6$\pm$33.6}& 13.8$\pm$4.2& \textbf{16.3$\pm$4.3}& 15.9$\pm$5.1& 14.6$\pm$3.7\\ 
&(-53.7)&(-46.0)&(-13.8)& \textbf{(-12.1)}&(-83.6)& \textbf{(-81.1)}&(-81.5)&(-82.8)\\ 
\multirow{2}{*}{pendigits}	& 64.0$\pm$9.3& 85.9$\pm$6.6& \textbf{99.1$\pm$0.5}& 98.9$\pm$0.4& 77.9$\pm$6.8& 83.3$\pm$4.7& 99.2$\pm$0.6& \textbf{99.7$\pm$0.1}\\ 
&(-33.1)&(-11.2)& \textbf{(+2.0)}&(+1.8)&(-21.3)&(-15.9)&(+0.0)& \textbf{(+0.5)}\\  
\multirow{2}{*}{pima}	& 59.5$\pm$3.4& 60.6$\pm$2.6& \textbf{60.8$\pm$1.8}& \textbf{60.8$\pm$1.0}& 58.2$\pm$3.7& 59.0$\pm$1.4& \textbf{64.1$\pm$1.5}& 61.1$\pm$1.4\\ 
&(-2.2)&(-1.1)& \textbf{(-0.9)}&\textbf{(-0.9)}&(-2.1)&(-1.3)& \textbf{(+3.8)}&(+0.8)\\ 
\multirow{2}{*}{satellite}	& 80.9$\pm$0.4& 82.2$\pm$0.3& 82.6$\pm$0.4& \textbf{82.9$\pm$0.3}& 78.5$\pm$1.2& 78.3$\pm$1.0& 79.3$\pm$0.9& \textbf{79.5$\pm$1.0}\\ 
&(-1.5)&(-0.2)&(+0.2)& \textbf{(+0.5)}&(-6.7)&(-6.9)&(-5.9)& \textbf{(-5.7)}\\ 
\multirow{2}{*}{satimage}	& 92.3$\pm$2.1& \textbf{99.7$\pm$0.1}& \textbf{99.7$\pm$0.1}& \textbf{99.7$\pm$0.1}& 89.8$\pm$1.6& 99.6$\pm$0.2& \textbf{99.7$\pm$0.1}& \textbf{99.7$\pm$0.1}\\ 
&(-7.5)& \textbf{(-0.1)}&\textbf{(-0.1)}&\textbf{(-0.1)}&(-9.9)&(-0.1)& \textbf{(+0.0)}&\textbf{(+0.0)}\\ 
\multirow{2}{*}{seismic}	& 51.6$\pm$0.5& 49.7$\pm$2.0& 50.3$\pm$3.0& \textbf{55.6$\pm$3.8}& 56.9$\pm$2.7& 58.4$\pm$2.3& \textbf{68.0$\pm$1.9}& 66.3$\pm$1.6\\ 
&(-1.3)&(-3.2)&(-2.6)& \textbf{(+2.7)}&(-6.5)&(-5.0)& \textbf{(+4.6)}&(+2.9)\\ 
\multirow{2}{*}{shuttle}	& 99.7$\pm$0.1& \textbf{99.8$\pm$0.1}& 99.7$\pm$0.1& 99.7$\pm$0.1& \textbf{99.7$\pm$0.1}& 99.6$\pm$0.0& \textbf{99.7$\pm$0.0}& \textbf{99.7$\pm$0.1}\\ 
&(+0.1)& \textbf{(+0.2)}&(+0.1)&(+0.1)& \textbf{(-0.3)}&(-0.4)&\textbf{(-0.3)}&\textbf{(-0.3)}\\ 
\multirow{2}{*}{speech}	& 48.6$\pm$1.2& 53.2$\pm$1.4& 78.8$\pm$3.0& \textbf{85.5$\pm$1.6}& 17.1$\pm$1.9& 21.8$\pm$1.5& \textbf{24.2$\pm$1.3}& 18.0$\pm$1.9\\ 
&(-13.9)&(-9.3)&(+16.3)& \textbf{(+23.0)}&(-41.3)&(-36.6)& \textbf{(-34.2)}&(-40.4)\\ 
\multirow{2}{*}{thyroid}	& 94.3$\pm$1.2& 96.4$\pm$0.3& 99.1$\pm$0.2& \textbf{99.3$\pm$0.2}& 96.0$\pm$0.9& 97.7$\pm$0.3& \textbf{99.4$\pm$0.2}& 99.2$\pm$0.3\\ 
&(-3.9)&(-1.8)&(+0.9)& \textbf{(+1.1)}&(-2.4)&(-0.7)& \textbf{(+1.0)}&(+0.8)\\ 
\multirow{2}{*}{vertebral}	& 54.8$\pm$4.6& 55.3$\pm$4.3& 47.9$\pm$12.0& \textbf{59.2$\pm$9.8}& 43.3$\pm$1.5& \textbf{50.5$\pm$2.7}& 45.6$\pm$5.7& 46.8$\pm$4.9\\ 
&(-5.0)&(-4.5)&(-11.9)& \textbf{(-0.6)}&(-10.5)& \textbf{(-3.3)}&(-8.2)&(-7.0)\\ 
\multirow{2}{*}{vowels}	& 87.6$\pm$2.2& 92.6$\pm$3.5& \textbf{96.3$\pm$1.9}& 92.7$\pm$2.7& 91.0$\pm$2.6& 95.6$\pm$2.0& \textbf{99.2$\pm$0.3}& 98.3$\pm$0.6\\ 
&(-10.4)&(-5.4)& \textbf{(-1.7)}&(-5.3)&(-7.9)&(-3.3)& \textbf{(+0.3)}&(-0.6)\\ 
\multirow{2}{*}{wbc}	& 81.2$\pm$7.0& 88.5$\pm$5.0& \textbf{94.9$\pm$2.2}& 93.4$\pm$2.4& 86.3$\pm$2.0& 86.8$\pm$1.1& \textbf{91.5$\pm$1.1}& 91.0$\pm$0.5\\ 
&(-11.6)&(-4.3)& \textbf{(+2.1)}&(+0.6)&(-4.6)&(-4.1)& \textbf{(+0.6)}&(+0.1)\\ 
\multirow{2}{*}{wine}	& 64.3$\pm$14.4& 93.1$\pm$7.7& 99.6$\pm$0.1& \textbf{99.8$\pm$0.1}& 49.9$\pm$12.6& 54.6$\pm$8.3& 99.7$\pm$0.7& \textbf{100$\pm$0.0}\\ 
&(-35.4)&(-6.6)&(-0.1)& \textbf{(+0.1)}&(-48.6)&(-43.9)&(+1.2)& \textbf{(+1.5)}\\ 
\hline
	\end{tabular}
	}
	%\vspace{-5pt}
\end{table*}

==> Latent Outlier Exposure-ICML2022/tables/video_results.tex <==
\begin{table}[t!]
%\vspace{-5pt}
    %\small
	\caption{AUC ($\%$) for different contamination ratios for a video frame anomaly detection benchmark proposed in \citep{pang2020self}. LOE$_S$ (proposed) achieves state-of-the-art performance.}
	\label{tab:video_results}
	\centering
	\vspace{2pt}
 	\resizebox{\linewidth}{!}{
	\begin{tabular}{l|ccc}
        \hline
        Method    &\multicolumn{3}{c}{Contamination Ratio} \\
		     & 10\%   & 20\%  & 30\%$^*$ \\
		\hline
		\citep{tudor2017unmasking} &- &- &68.4 \\
		\citep{liu2018classifier} &- &- &69.0 \\
		\citep{del2016discriminative} &- &- &59.6 \\
		\citep{sugiyama2013rapid} &55.0 &56.0 &56.3 \\
		\citep{pang2020self} &68.0 &70.0 &\textbf{71.7} \\
        Blind &85.2$\pm$1.0 &76.0$\pm$2.7 &66.6$\pm$2.6 \\
        Refine & 82.7$\pm$1.5 &74.9$\pm$2.4 &69.3$\pm$0.7 \\
        LOE$_H$ (ours) & 82.3$\pm$1.6 &59.6$\pm$3.8 &56.8$\pm$9.5 \\
        LOE$_S$ (ours)& \textbf{86.8$\pm$1.2} &\textbf{79.2$\pm$1.3} &\textbf{71.5$\pm$2.4} \\
        % Blind &85.2$\pm$1.0 (-6.3) &76.0$\pm$2.7 (-15.5) &66.6$\pm$2.6 (-24.9) \\
        % Refine & 82.7$\pm$1.5 (-8.8) &74.9$\pm$2.4 (-16.6) &69.3$\pm$0.7 (-22.2) \\
        % LOE-H & 82.3$\pm$1.6 (-9.2) &59.6$\pm$3.8 (-31.9) &56.8$\pm$9.5 (-34.7) \\
        % LOE-S & \textbf{86.8$\pm$1.2 (-4.7)} &\textbf{79.2$\pm$1.3 (-12.3)} &\textbf{71.5$\pm$2.4 (-20.0)} \\
        \hline
        \multicolumn{4}{l}{{ 
         $^*$Default setup in \citep{pang2020self}, corresponding to $\alpha_0\approx 30 \%$.
        }}\\
        %\multicolumn{4}{l}{{\tiny 
        %  $^\flat$\citep{tudor2017unmasking},
        %  $^\natural$\citep{liu2018classifier},
        %  $^\P$\citep{del2016discriminative},
        %}}\\
        %\multicolumn{4}{l}{{\tiny 
        %  $^\S$\citep{liu2012isolation, sugiyama2013rapid}, %$^\sharp$\citep{pang2020self}
        %}}
	\end{tabular}
 	}
%	\vspace{-5pt}
\end{table}

==> Latent Outlier Exposure-ICML2022/theory.tex <==
\section{Theory}

As follows, we will start by explaining our basic setup as well as our optimization objective. We will show that our approach is indeed an EM scheme in the classical sense and can be shown to optimize the target of interest. The analysis draws on a continuous relaxation of a discrete optimization problem. [Note that the current version may contain sign errors.]

\paragraph{Problem setup.} As follows, denote $L_n(x_i)$ and $L_a(x_i)$ our loss functions for normal and anomalous data, respectively. Since our training data contains both normal data $(x_i, y_i=0)$ and anomalies $(x_i, y_i=1)$, our goal is to minimize the loss function under the assumption of the best configuration of assignment variables $y_i$. This allows us to define a joint loss over ${\bf x}$ and ${\bf y}$ as follows:
%
\begin{align}
    L({\bf x},{\bf y}) = \sum_{i=1}^N y_i L_n(x_i) + (1-y_i) L_a(x_i).
\end{align}
%
When optimizing this loss function, we assume that the fraction of normal over anomalous data is roughly given by a fraction $0 \leq \alpha \leq 1$. Our optimization problem can hence be written as
\begin{align}
    \min_\theta L^\theta({\bf x}) = \min_\theta \min_{\bf y} L({\bf x},{\bf y}) \; \textrm{s.th.} \; \frac{\#\{y_i=0\}}{\#\{y_i\}} = \alpha.
\end{align}
That is, we ask for the optimal assignments of binary labels to training data and optimize the loss accordingly over its parameters. 
To simplify the notation, we drop the constraint on the  fraction of normal data $\alpha$, but we will get back to it. 
\paragraph{Proposed scheme.} As follows, we proposed a scheme to optimize the loss function. We will prove the correctness of the scheme later on.

We consider the following binary classifier,
\begin{align}
    p_\theta(y_i=0 | x_i) =
    \begin{cases}
    1 & L^\theta_n(x_i)  < L^\theta_a(x_i) + C_\alpha \\ 0 & \textrm{else}.
    \end{cases}
\end{align}
Note that the classifier is currently deterministic, but we consider probabilistic extensions below. Importantly, the behavior of the classifier can be steered with the parameter $C_\alpha$. We will discuss its connection to the assumed rate of normal data $\alpha$ below. Note that, alternatively to selecting a threshold $C$, one can also select C so that a fixed fraction of datapoints are classified as normal or anomalous, i.e., choose $C_\alpha$ such that $E_{x_i,y_i}[p_\theta(y_i=0 | x_i)] = \alpha$. 

In order to optimize the loss function, we follow the following scheme:
\begin{align}
    \theta_{t+1} &= \arg \min_\theta Q(\theta | \theta_t)\\    Q(\theta | \theta_t) & = E_{p_{\theta_t}({\bf y}|{\bf x})}[L({\bf x},{\bf y})]\\
    & = E_{p_{\theta_t}({\bf y}|{\bf x})}[ \sum_{i=1}^N y_i L^\theta_n(x_i) + (1-y_i)L^\theta_a(x_i)].\nonumber
\end{align}
That is, we iterate between both update steps: (1) minimizing the expected loss $Q$ (expectation under $p_{\theta_t}({\bf y}|{\bf x})$) over model parameters $\theta$, and (2) re-computing the loss by re-estimating the binary variables $y_i$ using the updated classifier. 
These updates are inspired by the EM algorithm [CITE: Dempster 1977] and shall be motivated below.

\paragraph{Correctness of the scheme.}

As follows, we show that the proposed scheme above can be derived from a smoothed relaxation of the discrete optimization problem over ${\bf y}$. In more detail, we draw a connection to the EM algorithm and justify the update scheme. This is possible even without requiring the loss function $L({\bf x},{\bf y})$ to have a probabilistic interpretation. 

For the following analysis, it will be more intuitive to think about \emph{maximizing} the negative loss than to minimize the loss. 
That is, our objective of maximization is 
\begin{align}
-L^\theta({\bf x}) & = \max_{{\bf y} \in \{0,1\}^N}-L^\theta({\bf x},{\bf y}) \\ 
    & = \sum_{i=1}^N \max \{-L^\theta_n(x_i), -L^\theta_a(x_i)\} \\
     & \stackrel{\beta \rightarrow \infty}{=}\sum_{i=1}^N \beta^{-1}\log (e^{-\beta L^\theta_n(x_i)} + e^{-\beta L^\theta_a(x_i)})\\
     & =  \beta^{-1}\log \prod_{i=1}^N(e^{-\beta L^\theta_n(x_i)} + e^{-\beta L^\theta_a(x_i)}).
\end{align}
We have just shown that a continuous relaxation of the problem formulation exists, where the maximization operation is replaced by the sum of two exponential functions. For the following analysis, we consider a finite $\beta>0$. Note that only $\beta \rightarrow \infty$ yields the exact identity.

We will sometimes suppress the dependence of different expressions on $\beta$ in the notation for now and consider it to be a finite but very large number. We can now formally \emph{define} an un-normalized probability $p_\theta({\bf x}|{\bf y}) = \prod_{i=1}^N p_\theta(x_i | y_i)$, over data given the binary labels, where
\begin{align}
    p_\theta(x_i|y_i) = \beta^{-1} \times
    \begin{cases}
    e^{-\beta L^\theta_n(x_i)} & y_i = 0 \\ e^{-\beta L^\theta_a(x_i)} & y_i = 1
    \end{cases}
\end{align}
Equivalently, we can write
\begin{align}
    p_\theta(x_i|y_i) = \beta^{-1} \exp \{-y_i \beta L^\theta_a(x_i) - (1-y_i) \beta L^\theta_n(x_i)\}.
\end{align}
For now, we don't worry about the fact that these probabilities are not normalized (or even \emph{normalizable})--this will not be required in our derivation. For the purpose of this section, they are just functions. Yet, interpreting them as probabilities can be useful to understand the analogy to the EM algorithm. 

We can equip this un-normalized "likelihood" distribution with a Bernoulli prior,
\begin{align}
    p_\theta(y_i) = \exp \{y_i \log \alpha + (1-y_i) \log (1-\alpha)\}.
\end{align}
The resulting joint distribution is
\begin{multline}
    p_\theta(x_i,y_i) = \exp \{y_i (\log \alpha - \beta L^\theta_a(x_i)) \\ + (1-y_i) (\log (1-\alpha) - \beta L^\theta_n(x_i))\}.
\end{multline}

The resulting posterior distribution is
\begin{align}
    p(y_i=0|x_i) = \frac{e^{-\beta L_n(x_i) + \log \alpha}}{e^{-\beta L_n(x_i)+ \log \alpha}+e^{-\beta L_a(x_i) + \log (1-\alpha)}}
\end{align}
We stress that while the joint distribution is not normalized, the posterior is normalized by construction.

As follows, we define the log-odds as $C_\alpha = \log \alpha - \log (1-\alpha)$. 
For $\beta \rightarrow \infty$, the posterior becomes deterministic and results in 
\begin{align}
    y_i | x_i = 
    \begin{cases}
    0 & L_n(x_i)  < L_a(x_i) + C \\ 1 & \textrm{else}.
    \end{cases}
\end{align}
Note that by construction, the posterior reflects exactly the behavior of our classifier that we introduced in the EM scheme. Using the terminology introduced above, our scheme translates (in the case of finite $beta$) into
\begin{align}
    \theta_{t+1} &= \arg \max_\theta Q(\theta | \theta_t)\\    Q(\theta | \theta_t) & = E_{p_{\theta_t}(y|x)}[\log p_{\theta}(x,y)]
\end{align}
This is the classical definition of EM according to \citep{dempster1977maximum, little1987statistical}. As shown by \citet{little1987statistical}\footnote{see also "proof of correctness" in Wikipedia article on EM}, every update improves the model's marginal likelihood. This means that it is a coordinate update scheme that results in a local optimum of the continuous relaxation of our loss. 
 
Note that this proof doesn't require the likelihood function be normalized (this still needs to be checked). Hence, our scheme is correct even if $L_n$ and $L_a$ don't have probabilistic interpretations. 

==> tables/negative_losses.tex <==
\begin{table}[ht]
%\vspace{-6pt}
	\caption{$\La$ for various anomaly detectors.}
	\label{tab:anomaly loss}
	\centering
	\vspace{3pt}
%	\resizebox{\linewidth}{!}{
	\begin{tabular}{l|c}
        \hline
        & $\La$\\
        \hline
         \vspace{5pt}       
        MHRot& 
   $ \sum_{c=1}^{|\mathcal{T}|}\sum_{l=1}^3 \text{CE}(\mathcal{U}, p_l(\cdot \mid f,T_c(\x)))$\\
        \vspace{5pt}
        NTL& $-\sum_{k=1}^K \log (1-p_k(x\mid f,\mathcal{T}))$\\
        \vspace{5pt}
        ICL& $-\sum_{k=1}^K \log (1-p_k(x\mid f,g,\mathcal{T}))$\\
        \vspace{5pt}
        DSVDD & $1/||f(x)-c||^2 $\\
        \hline
	\end{tabular}
%	}
	\vspace{-5pt}
\end{table}

==> theory.tex <==
\section{Theory}

As follows, we will start by explaining our basic setup as well as our optimization objective. We will show that our approach is indeed an EM scheme in the classical sense and can be shown to optimize the target of interest. The analysis draws on a continuous relaxation of a discrete optimization problem. [Note that the current version may contain sign errors.]

\paragraph{Problem setup.} As follows, denote $L_n(x_i)$ and $L_a(x_i)$ our loss functions for normal and anomalous data, respectively. Since our training data contains both normal data $(x_i, y_i=0)$ and anomalies $(x_i, y_i=1)$, our goal is to minimize the loss function under the assumption of the best configuration of assignment variables $y_i$. This allows us to define a joint loss over ${\bf x}$ and ${\bf y}$ as follows:
%
\begin{align}
    L({\bf x},{\bf y}) = \sum_{i=1}^N y_i L_n(x_i) + (1-y_i) L_a(x_i).
\end{align}
%
When optimizing this loss function, we assume that the fraction of normal over anomalous data is roughly given by a fraction $0 \leq \alpha \leq 1$. Our optimization problem can hence be written as
\begin{align}
    \min_\theta L^\theta({\bf x}) = \min_\theta \min_{\bf y} L({\bf x},{\bf y}) \; \textrm{s.th.} \; \frac{\#\{y_i=0\}}{\#\{y_i\}} = \alpha.
\end{align}
That is, we ask for the optimal assignments of binary labels to training data and optimize the loss accordingly over its parameters. 
To simplify the notation, we drop the constraint on the  fraction of normal data $\alpha$, but we will get back to it. 
\paragraph{Proposed scheme.} As follows, we proposed a scheme to optimize the loss function. We will prove the correctness of the scheme later on.

We consider the following binary classifier,
\begin{align}
    p_\theta(y_i=0 | x_i) =
    \begin{cases}
    1 & L^\theta_n(x_i)  < L^\theta_a(x_i) + C_\alpha \\ 0 & \textrm{else}.
    \end{cases}
\end{align}
Note that the classifier is currently deterministic, but we consider probabilistic extensions below. Importantly, the behavior of the classifier can be steered with the parameter $C_\alpha$. We will discuss its connection to the assumed rate of normal data $\alpha$ below. Note that, alternatively to selecting a threshold $C$, one can also select C so that a fixed fraction of datapoints are classified as normal or anomalous, i.e., choose $C_\alpha$ such that $E_{x_i,y_i}[p_\theta(y_i=0 | x_i)] = \alpha$. 

In order to optimize the loss function, we follow the following scheme:
\begin{align}
    \theta_{t+1} &= \arg \min_\theta Q(\theta | \theta_t)\\    Q(\theta | \theta_t) & = E_{p_{\theta_t}({\bf y}|{\bf x})}[L({\bf x},{\bf y})]\\
    & = E_{p_{\theta_t}({\bf y}|{\bf x})}[ \sum_{i=1}^N y_i L^\theta_n(x_i) + (1-y_i)L^\theta_a(x_i)].\nonumber
\end{align}
That is, we iterate between both update steps: (1) minimizing the expected loss $Q$ (expectation under $p_{\theta_t}({\bf y}|{\bf x})$) over model parameters $\theta$, and (2) re-computing the loss by re-estimating the binary variables $y_i$ using the updated classifier. 
These updates are inspired by the EM algorithm [CITE: Dempster 1977] and shall be motivated below.

\paragraph{Correctness of the scheme.}

As follows, we show that the proposed scheme above can be derived from a smoothed relaxation of the discrete optimization problem over ${\bf y}$. In more detail, we draw a connection to the EM algorithm and justify the update scheme. This is possible even without requiring the loss function $L({\bf x},{\bf y})$ to have a probabilistic interpretation. 

For the following analysis, it will be more intuitive to think about \emph{maximizing} the negative loss than to minimize the loss. 
That is, our objective of maximization is 
\begin{align}
-L^\theta({\bf x}) & = \max_{{\bf y} \in \{0,1\}^N}-L^\theta({\bf x},{\bf y}) \\ 
    & = \sum_{i=1}^N \max \{-L^\theta_n(x_i), -L^\theta_a(x_i)\} \\
     & \stackrel{\beta \rightarrow \infty}{=}\sum_{i=1}^N \beta^{-1}\log (e^{-\beta L^\theta_n(x_i)} + e^{-\beta L^\theta_a(x_i)})\\
     & =  \beta^{-1}\log \prod_{i=1}^N(e^{-\beta L^\theta_n(x_i)} + e^{-\beta L^\theta_a(x_i)}).
\end{align}
We have just shown that a continuous relaxation of the problem formulation exists, where the maximization operation is replaced by the sum of two exponential functions. For the following analysis, we consider a finite $\beta>0$. Note that only $\beta \rightarrow \infty$ yields the exact identity.

We will sometimes suppress the dependence of different expressions on $\beta$ in the notation for now and consider it to be a finite but very large number. We can now formally \emph{define} an un-normalized probability $p_\theta({\bf x}|{\bf y}) = \prod_{i=1}^N p_\theta(x_i | y_i)$, over data given the binary labels, where
\begin{align}
    p_\theta(x_i|y_i) = \beta^{-1} \times
    \begin{cases}
    e^{-\beta L^\theta_n(x_i)} & y_i = 0 \\ e^{-\beta L^\theta_a(x_i)} & y_i = 1
    \end{cases}
\end{align}
Equivalently, we can write
\begin{align}
    p_\theta(x_i|y_i) = \beta^{-1} \exp \{-y_i \beta L^\theta_a(x_i) - (1-y_i) \beta L^\theta_n(x_i)\}.
\end{align}
For now, we don't worry about the fact that these probabilities are not normalized (or even \emph{normalizable})--this will not be required in our derivation. For the purpose of this section, they are just functions. Yet, interpreting them as probabilities can be useful to understand the analogy to the EM algorithm. 

We can equip this un-normalized "likelihood" distribution with a Bernoulli prior,
\begin{align}
    p_\theta(y_i) = \exp \{y_i \log \alpha + (1-y_i) \log (1-\alpha)\}.
\end{align}
The resulting joint distribution is
\begin{multline}
    p_\theta(x_i,y_i) = \exp \{y_i (\log \alpha - \beta L^\theta_a(x_i)) \\ + (1-y_i) (\log (1-\alpha) - \beta L^\theta_n(x_i))\}.
\end{multline}

The resulting posterior distribution is
\begin{align}
    p(y_i=0|x_i) = \frac{e^{-\beta L_n(x_i) + \log \alpha}}{e^{-\beta L_n(x_i)+ \log \alpha}+e^{-\beta L_a(x_i) + \log (1-\alpha)}}
\end{align}
We stress that while the joint distribution is not normalized, the posterior is normalized by construction.

As follows, we define the log-odds as $C_\alpha = \log \alpha - \log (1-\alpha)$. 
For $\beta \rightarrow \infty$, the posterior becomes deterministic and results in 
\begin{align}
    y_i | x_i = 
    \begin{cases}
    0 & L_n(x_i)  < L_a(x_i) + C \\ 1 & \textrm{else}.
    \end{cases}
\end{align}
Note that by construction, the posterior reflects exactly the behavior of our classifier that we introduced in the EM scheme. Using the terminology introduced above, our scheme translates (in the case of finite $beta$) into
\begin{align}
    \theta_{t+1} &= \arg \max_\theta Q(\theta | \theta_t)\\    Q(\theta | \theta_t) & = E_{p_{\theta_t}(y|x)}[\log p_{\theta}(x,y)]
\end{align}
This is the classical definition of EM according to \citep{dempster1977maximum, little1987statistical}. As shown by \citet{little1987statistical}\footnote{see also "proof of correctness" in Wikipedia article on EM}, every update improves the model's marginal likelihood. This means that it is a coordinate update scheme that results in a local optimum of the continuous relaxation of our loss. 
 
Note that this proof doesn't require the likelihood function be normalized (this still needs to be checked). Hence, our scheme is correct even if $L_n$ and $L_a$ don't have probabilistic interpretations. 
